Making Auctions Robust to Aftermarkets

A prevalent assumption in auction theory is that the auctioneer has full control over the market and that the allocation she dictates is final. In practice, however, agents might be able to resell acquired items in an aftermarket. A prominent example is the market for carbon emission allowances. These allowances are commonly allocated by the government using uniform-price auctions, and firms can typically trade these allowances among themselves in an aftermarket that may not be fully under the auctioneer's control. While the uniform-price auction is approximately efficient in isolation, we show that speculation and resale in aftermarkets might result in a significant welfare loss. Motivated by this issue, we consider three approaches, each ensuring high equilibrium welfare in the combined market. The first approach is to adopt smooth auctions such as discriminatory auctions. This approach is robust to correlated valuations and to participants acquiring information about others' types. However, discriminatory auctions have several downsides, notably that of charging bidders different prices for identical items, resulting in fairness concerns that make the format unpopular. Two other approaches we suggest are either using posted-pricing mechanisms, or using uniform-price auctions with anonymous reserves. We show that when using balanced prices, both these approaches ensure high equilibrium welfare in the combined market. The latter also inherits many of the benefits from uniform-price auctions such as price discovery, and can be introduced with a minor modification to auctions currently in use to sell carbon emission allowances.

==> content/additional_example.tex <==
\section{Additional Example}
\label{apx:additional example}
% \begin{example}\label{exp:constrained demand}
% There are $m > 3$ units to be allocated and $2$ agents named $A,B$. 
% We assume that the 
% Agent $A$ has marginal value $2$ for the first unit, value uniformly sample from $[1,1.5]$ for the second unit, and $0$ for any subsequent units. 
% % That is, $v_A(S) = \min\{|S|,2\}$. 
% Agent $B$ has the following distribution over valuations.  She always has marginal value $2$ for the first unit acquired, then a value $z_B > 0$ for each subsequent unit acquired. 
% Here $z_B$ is a random variable drawn from a distribution with CDF $F(z) = 1-\frac{1}{1+(2m-1)z}$ for $z \in [0, 1)$ and $F(z) = z-\frac{1}{2m}$ for $z\in [1,1+\frac{1}{2m}]$. 
% Note that given buyer value with distribution $F$,
% the unique revenue maximizing price is $p=1$ with {expected revenue of} $p \cdot \Pr[z_B \geq p] = 1/(2m)$ {per-unit}.
% Agent $C$ has value $0$ for any number of units; we refer to agent $C$ as a \emph{speculator}.

% The primary auction will be a uniform-price auction with standard bidding.
% The auction is resolved by allocating units in order of bids (breaking ties in any arbitrary but consistent manner) until all units have been allocated.  The price $p$ per unit is set equal to the highest unallocated bid.  Each agent then pays $p$ per unit received.

% In the secondary market, the speculator $C$ can put some or all of the licenses that she has acquired in the auction up for sale, at a take-it-or-leave-it price of her choice. Agent $A$ has the first opportunity to purchase any (or all) of the licenses made available by $C$.  
% Then agent $B$ has the option to purchase any licenses that are still available.\footnote{A more general secondary market can allow all agents to offer acquired licenses for sale, not just agent $C$. The result presented extends to such more general version as well, but for simplicity we focus on a secondary market where only agent $C$ can sell.}
% \end{example}


==> content/conclusion.tex <==
\section{Conclusions and Discussions}
\label{sec:conclusion}

\mbc{this is OLD. Rewrite with policy implications}

In this paper, we have shown that although the equilibrium welfare may decrease in the presence of information acquisition or secondary markets, 
the worst case guarantee will not decrease if the mechanisms adopted in the auction is smooth. 
With this in mind, one might wonder if the result can be extended to mechanisms that are only smooth under some equilibrium refinement (like undominated strategies).
However, as we illustrated in \Cref{sec:refine}, 
the smoothness result under refinement cannot be generalized to the setting with secondary markets even if there is no information acquisition, 
since agents can benefit from speculation in the combined market. 
Moreover, for the first-price auction in the single-item settings with two-agent having i.i.d. distributions, 
we show that information acquisition can still lead to efficiency loss
while all equilibria are efficient
under natural assumptions on the secondary markets.


Our paper provides a preliminary understanding of the welfare guarantees when agents can acquire costly information and the auction is followed by secondary markets. 
%there exist secondary markets. 
Note that our techniques and results are not limited to the exact model we have presented in this paper. 
For example, 
the reduction framework we introduced in \Cref{sec:smooth} extends easily when the agents 
discount the value for the items they acquire in the secondary markets. 
This discounting behavior is natural to consider if we view the secondary markets as a place where agents can trade used items, 
and people usually value less for the used items. 

Another example is to generalize our framework to settings 
where the exact smooth framework does not deliver the tightest analysis, 
e.g., simultaneous first-price auction for subadditive valuations \citep{feldman2013simultaneous}
and sequential first-price auction for unit-demand valuations \citep{syrgkanis2012bseq}. 
For those setting, the smooth parameter is large while the price of anarchy is small.  
The idea for showing small price of anarchy resembles the smooth analysis, 
where for the given mechanisms, 
there exist deviating strategies for each agent with sufficiently large utility
and hence the total utilities of all agent are sufficiently high under any equilibrium. 
The latter guarantees small price of anarchy for the given mechanism. 
One can imitate their proof step by step and show that the price of anarchy results for those settings extend when agents can acquire costly information
and there is a secondary market satisfying voluntary participation and weak budget balance. 


There are also a lot of interesting open questions remaining. 
In the symmetric case, we only prove the efficiency result for two agents when all agents adopt monotone bids. 
A possible direction is to generalize the result to three or more agents, and without any assumption on the strategies. 
In our work, we only show that the price of anarchy cannot increase when the mechanism is smooth. 
It would be interesting to see if one can design specific information acquisition structures or specific secondary markets such that the price of anarchy of the combined market strictly decreases 
compared to the setting with standalone auction.


==> content/notes.tex <==
\section{Summary}
\begin{enumerate}
\item Secondary market may decreases the equilibrium welfare \citep{hafalir2009revenue}.
\item The decrease in welfare may due to the speculation behavior of the agents \citep[e.g.,][]{garratt2006speculation}. 
The speculation has more severe impact on efficiency when considering second price auction.


\item (Section PoA using smooth argument:) In addition, if the auction is smooth, 
even though the expected welfare may decrease, 
the worst case guarantee (over both the valuation distribution and the equilibrium selection) does not, 
i.e., PoA does not increase. 
This holds for any number of bidders.
Moreover, this result is robust to the information revealed and the transaction rules in secondary markets.  Also extends to smooth auctions for multiple items.  Discuss subtleties around equilibrium refinements (compare discriminatory pricing vs uniform pricing).  \bjl{Todo: extended refinement that gets back a positive result?}



\item (Section 1 item - Subsection 1) However, for first price or all pay auctions with two bidders, 
the impact of speculation on efficiency is eliminated when the distributions are symmetric.  This holds for a general class of secondary markets; prior work had established this for specific forms of secondary market.  \bjl{Todo: $3$ or more bidders?}

\item (Section 1 item - Subsection 2) For revenue maximization, 
we show that if the bids are not revealed in the secondary market, 
the first price auction or second price auction with anonymous reserve is 2.62 approximation to the optimal revenue. 

\item \mbc{Mainly about many item case (appendix):} Finally, since one effect on the decrease in equilibrium is the coordination of agents in the secondary markets, 
we consider the single strategic agent setting and show that the equilibrium welfare does not decrease. 


\end{enumerate}

\mbc{Remarks:
\begin{itemize}
    \item We should emphasize the fact we have results for $n>2$ buyers, while most prior results are only for $n=2$ buyers.  
    \item counterexample for 3 iid bidders?
\end{itemize}
}


\section{Setting}
The seller tries to sell a set of items to $n$ agents 
among the set of feasible allocations $\feasibles$. 
% We assume $\feasibles$ is a finite set. 
Let $\types = \times_i\types_i$ be the type space of the agents
and $\dist$ be the prior distribution over the type space.
For any agent $i$, her type $\type_i\in \types_i$ is her private information
and the marginal distribution of her private type is denoted by $\dist_i$.
%$(\types_i, \borels_i, \dist_i)$ be a probability space 
% where $\types_i$ is the type space of agent $i$, 
% and $\borels_i$ is a $\sigma$-algebra of $\types_i$. 
% Let $\dist = \times_i \dist_i$ be the product measure. 
% The agent $i$ have private type $\type_i \in \types_i$ 
% where $\type_i \sim \dist_i$
% and $\dist_i$ is a distribution over type space $\types_i$.
% Let $\dist = \times_i \dist_i$ be the joint distribution
% and $\dists$ be the set of possible distributions. 
Let $\val_i(\alloc; \type_i)$ be the public valuation function of agent $i$
given allocation $\alloc \in \feasibles$ and type $\type_i$,
and her utility given allocation $\alloc$
and payment $\pay_i$
is $u_i(\alloc, \pay_i; \type_i) = \val_i(\alloc; \type_i) - \pay_i$.
Moreover, all agents have von Neumann–Morgenstern expected utility for randomized outcomes. 
Note that here we allow agents to have externalities of the valuation on the allocation. 
In this auction environment, 
the seller adopts the mechanism 
$\mech_1: \actions^F \to \Delta(\feasibles \times \reals^n)$, 
where $\actions^F = \times_i \actions^F_i$, 
and $\actions^F_i$ is the action space of agent $i$ in the auction.
To simplify the notation, 
let $\alloc^{\mech}, \pay^{\mech}$
be the allocation and payment rule given mechanism~$\mech$.
% and $\kappa$ is the randomization device of mechanism~$\mech_1$. 
% We assume that for each $i$, there exists $\alloc^i \in \feasibles$ such that $\val_i(\alloc; \type_i) = 0$ for all $\type_i$, 
% and there exists an action $\action^F_i \in \actions^F_i$
% such that $\mech_1(\action^F_i, \action^F_{-i}) = $

After the auction, there is a secondary market $\mech_2: \actions^S \times \feasibles \to \Delta(\feasibles \times \reals^n)$
where agents can re-trade their items after participating in mechanism $\mech_1$.\footnote{In the definition of the secondary market, 
it is implicitly assumed that the allocation realized in the auction environment is publicly revealed before the secondary market. 
This can be relaxed such that each agent only observes her own allocation. 
In this scenario, the agent will maximize her expected utility by taking expectation over the randomness of the allocation. 
Our results in this paper carries through with this generalization, 
which will not be formally proved in later sections. } 
Let $\mech_C$ be the combined mechanism of $\mech_1$ and $\mech_2$.
We assume that the secondary market satisfies two nature properties, 
voluntary participation and weak budget balance. 
\begin{definition}
A secondary market $\mech_2$ satisfies \emph{voluntary participation} if for each agent $i$ and all types $\type_i$, 
there exists an action $\action^S_i \in \actions^S_i$
such that $\val_i(\alloc; \type_i) \leq u_i(\mech_2(\alloc, (\action^S_i, \action^S_{-i}));\type_i)$ 
for any allocation $\alloc$
and any action profile $\action^S_{-i}$.
\end{definition}

\begin{definition}
A secondary market $\mech_2$ satisfies \emph{weak budget balance} if 
$\sum_i \pay^{\mech_2}_i(\action^S, \alloc) \geq 0$
for any action $\action^S\in \actions^S$ and feasible allocation $\alloc\in \feasibles$.
\end{definition}

% Note that if in addition mechanism $\mech_1$ satisfies voluntary participation, 
% the combined mechanism $\mech_C$ satisfies voluntary participation as well.

% In general we have voluntary participation for mechanism $\mech_2$. 
% That is, that for each $i$ and all types $\type_i$, there exists an action $\action^S_i \in \actions^S_i$
% such that $\val_i(\alloc; \type_i) \leq u_i(\mech_2(\alloc, (\action^S_i, \action^S_{-i}));\type_i)$ for all allocation $\alloc$
% and all action profile $\action^S_{-i}$.
% Let $\mech_C$ be the combined mechanism.
% Note the if in addition mechanism $\mech_1$ satisfies voluntary participation, 
% the combined mechanism $\mech_C$ satisfies voluntary participation as well.
% Let $\alloc^{\mech}, \pay^{\mech}$
% be the allocation and payment rule given mechanism~$\mech$. 
% Note that in this paper, we model the secondary market as a stage where agents can renegotiate and trade the allocation with transfers among themselves. 
% Thus we assume that $\mech_2$ is budget balanced, that is, $\sum_i \pay^{\mech_2}_i(\action^S, \alloc) = 0$
% for all $\action^S\in \actions^S$ and $\alloc\in \feasibles$.


For any type profile $\type$, 
let $\wel(\type;\val,\feasibles)$ be the corresponding optimal welfare
given the valuation functions $\val$ and feasibility constraint $\feasibles$. 
Let $\wel(\dist; \val, \feasibles) = \expect[\type\sim\dist]{\wel(\type;\val,\feasibles)}$ be the expected optimal welfare.
When functions $\val$ and $\feasibles$ are clear from the context, 
we omit it in the notation and use $\wel(\type), \wel(\dist)$ to denote the optimal and expected optimal welfare. 
By slightly overloading the notation, 
we also denote $\wel(\mech, \strategy, \dist)$ 
as the expected welfare obtained in mechanism $\mech$ using strategy profile $\strategy$. 
Let 
\begin{align*}
\poa(\mech, \dists) = \max_{\dist\in \dists} 
\frac{\wel(\dist)}{\min_{\strategy\in \BNE(\dist, \mech)}\{\wel(\mech, \strategy, \dist)\}}
\end{align*}
be the price of anarchy of mechanism $\mech$ within the family of distributions $\dists$.

Similarly, for the revenue objective, 
by omitting the publicly known valuation functions $\val$ and feasibility constraint $\feasibles$ in the notation, 
given any mechanism $\mech$, we denote its revenue given action profile $\action$ by $\rev(\action;\mech)$,
and denote the expected revenue given type distribution~$\dist$
and equilibrium strategy $\strategy$
by $\rev(\mech, \strategy,\dist)$. 
The optimal revenue given distribution $\dist$
is defined as 
$\rev(\dist) = \max_{\mech\in \mathbb{M},\strategy\in \BNE(\dist, \mech)}\{\rev(\mech, \strategy, \dist)\}$
where $\mathbb{M}$ is the set of auction mechanisms satisfying voluntary participation
and there is no secondary market.
Then the price of anarchy for revenue is 
\begin{align*}
\poar(\mech, \dists) = \max_{\dist\in \dists} 
\frac{\rev(\dist)}{\min_{\strategy\in \BNE(\dist, \mech)}\{\rev(\mech, \strategy, \dist)\}}.
\end{align*} 
Note that in the definition of the price of anarchy for revenue, 
we only compare to the benchmark of optimal Bayesian revenue 
when there is no secondary markets. 
One interpretation for this benchmark is that it can be viewed as an upper bound on the max-min revenue of the seller, 
where the maximum is taken over the auction mechanism, 
and the minimum is taken over the secondary market
and the equilibrium selection. 
Another reason for this choice is that the optimal revenue with secondary markets might be too large to approximate 
if the valuation of the agents are revealed in the secondary markets, 
which is illustrated in \Cref{exp:large rev}. 


\section{Smooth Framework}
If the allocation of the agents is given as exogenous, 
any secondary market satisfying voluntary participation
only increases the expected welfare of the market. 
However, if the allocation is endogenous, 
i.e., if the format of the secondary market and agents behavior in it
may distort their incentives in participating the auction,
as illustrated in \citet{hafalir2009revenue}, 
the expected equilibrium welfare may decrease in the combined market. 
However, in this paper, 
we will show that the worst case welfare guarantees 
of several classical mechanisms (e.g., first price auction) will not decrease
in the combined market
if they satisfy certain smooth properties. 


In \citet{roughgarden2012price, syrgkanis2013composable}, the authors developed the smoothness framework for analyzing the price of anarchy for auction environments. 
In this section, we show that the smoothness property is preserved for the combined market 
if the secondary market satisfying voluntary participation and weak budget balance. 

\begin{definition}[\citealp{syrgkanis2013composable}]\label{def:smooth}
For any $\lambda > 0,\mu\geq 1$, auction $\mech$ with action space $\actions$ is $(\lambda,\mu)$-smooth
if for any type profile $\type$,
there exists action distributions $\{\dista_i(\type)\}_{i\in [n]}$ such that 
for any action profile $\action\in \actions$, 
\begin{align*}
\sum_{i\in[n]} \expect[\action'_i\sim \dista_i(\type)]{\util_i(\mech(\action'_i, \action_{-i});\type_i)} \geq \lambda \wel(\type) - \mu \rev(\action;\mech)
\end{align*}
\end{definition}

\begin{theorem}[\citealp{roughgarden2012price, syrgkanis2013composable}]\label{thm:smooth imply poa}
Letting $\dists^{\Pi}$ be the family of all possible product distributions, 
for any $\lambda>0,\mu\geq 1$, 
if a mechanism $\mech$ is $(\lambda,\mu)$-smooth, 
then for any independent prior distribution of the types, 
the price of anarchy is at most $\frac{\mu}{\lambda}$, 
i.e., $\poa(\mech, \dists^{\Pi}) \leq \frac{\mu}{\lambda}$.
\end{theorem}

Next we illustrate how to generalizes the property of 
$(\lambda,\mu)$-smooth to combined markets. 
\begin{theorem}\label{thm:smooth}
For any $(\lambda,\mu)$-smooth mechanism $\mech_1$
and any secondary market mechanism $\mech_2$ satisfying voluntary participation and weak budget balance, 
the combined market $\mech_C = (\mech_1, \mech_2)$ is $(\lambda,\mu)$-smooth. 
\end{theorem}
\begin{proof}
Let $A^F, A^S$ be the action space of mechanisms $\mech_1, \mech_2$ respective, 
and $A^C = A^F \times A^S$ be the action space of the combined market. 
For each agent $i$, by voluntary participation, 
there exists action $\hat{a}^S_i \in A^S_i$ 
such that her payoff is at least her value of the initial allocation in the secondary market. 
Since mechanism $\mech_1$ is $(\lambda,\mu)$-smooth, 
for any type profile $\type$,
there exists action distributions $\{\dista^F_i(\type)\}_{i\in [n]}$ such that 
for any action profile $\action^F\in \actions^F$, 
\begin{align*}
\sum_{i\in[n]} \expect[\action'_i\sim \dista^F_i(\type)]{\util_i(\mech_1(\action'_i, \action^F_{-i});\type_i)} 
\geq \lambda \wel(\type) - \mu \rev(\action^F;\mech_1).
\end{align*}
For any type profile $\type$, let $\{\dista^C_i(\type)\}_{i\in [n]}$ be the distributions over actions $(\action^F_i, \hat{\action}^S_i)$ for each agent $i$
where $\action^F_i \sim \dista^F_i(\type)$. 
For any $\action^C \in \actions^C$, 
we have 
\begin{align*}
&\sum_{i\in[n]} \expect[\action'_i\sim \dista^C_i(\type)]{\util_i(\mech_C(\action'_i, \action^C_{-i});\type_i)} 
\geq \sum_{i\in[n]} \expect[\action'_i\sim \dista^F_i(\type)]{\util_i(\mech_1(\action'_i, \action^F_{-i});\type_i)} \\
&\geq \lambda \wel(\type) - \mu \rev(\action^F;\mech_1)
\geq \lambda \wel(\type) - \mu \rev(\action^C;\mech_C)
\end{align*}
where the first inequality holds by the definition of $\hat{\action}^S_i$
and the last inequality holds since mechanism $\mech_2$ is weakly budget balanced. 
\end{proof}

Note that \Cref{thm:smooth} does not depend on the details of the mechanism in the secondary market, 
or the information released in the secondary market. 
Moreover, it does not depends on the utility function of the agents. 
Thus, 
any $(\lambda,\mu)$-smooth mechanism guarantees robust welfare guarantee for any secondary markets satisfying voluntary participation and weak budget balance. 
Next we show some examples illustrating the power of the smoothness framework. 

First we consider the multi-item setting, 
where the feasibility constraint in this setting is that 
each item is allocated to at most one agent. 
We assume agents have submodular valuations, 
i.e., 
for any agent $i$, any type $\type_i$, 
any sets $X_1, X_2 \subseteq [n]$, we have 
$\val_i(X_1;\type_i) + \val_i(X_2;\type_i) \geq
\val_i(X_1\cap X_2;\type_i) + \val_i(X_1\cup X_2;\type_i)$.
Here $n$ is the number of items for the seller. 
Moreover, we assume agents have monotone valuations, 
i.e., 
for any agent $i$, any type $\type_i$, 
any sets $X_1\subseteq X_2 \subseteq [n]$, we have 
$\val_i(X_1;\type_i) \leq \val_i(X_2;\type_i)$.
In this setting, we consider the simultaneous first price auction, 
where each agent simultaneously announces her value for each item, 
the mechanism allocates each item to the highest bidder, 
and charges the agents their bids for each winning item. 

\begin{theorem}[\citealp{syrgkanis2013composable}]\label{thm:submodular}
For multi-item setting with monotone submodular valuations,
simultaneous first price auction is $(1-\sfrac{1}{e}, 1)$-smooth
and all-pay auction is $(1-\sfrac{1}{2}, 1)$-smooth. 
\end{theorem}

\begin{corollary}
For multi-item setting with monotone submodular valuations,
given any secondary market satisfying voluntary participation and weak budget balance,
the price of anarchy is at most $\sfrac{e}{(e-1)}$ for simultaneous first price auction 
and at most $2$ for all-pay auction.
\end{corollary}

Another example is the single-item multi-unit setting. 
Here we have $n$ units of the same item
and the feasibility constraint is that 
the total units sold to all agents is at most $n$. 
In addition to monotone submodular valuations, 
here we also consider monotone subadditive valuations,
i.e., 
for any agent $i$, any type $\type_i$, 
any sets $X_1, X_2 \subseteq [n]$, we have 
$\val_i(X_1;\type_i) + \val_i(X_2;\type_i) \geq
\val_i(X_1\cup X_2;\type_i)$.
The mechanism we adopt here is the discriminatory auction, 
a generalization of first price auction. 
Here each agent report her marginal value for each additional unit, 
the mechanism find the welfare maximization allocation, 
and charges the agents their bids for each additional unit they receive. 

\begin{theorem}[\citealp{de2013inefficiency}]\label{thm:submodular multi-unit}
For single-item multi-unit setting,
discriminatory auction is $(1-\sfrac{1}{e}, 1)$-smooth for monotone submodular valuations
and $(\frac{1}{2}(1-\sfrac{1}{e}), 1)$-smooth 
for monotone subadditive valuations. 
\end{theorem}

% \begin{theorem}[\citealp{feldman2013simultaneous}]\label{thm:subadditive}

% \end{theorem}

\begin{corollary}
For multi-unit setting,
given any secondary market satisfying voluntary participation and weak budget balance,
the price of anarchy of discriminatory auction is at most $\sfrac{e}{(e-1)}$ for monotone submodular valuations
and at most $\sfrac{2e}{(e-1)}$ for monotone subadditive valuations.
\end{corollary}


One limitation for \Cref{thm:smooth} and $(\lambda,\mu)$-smoothness
is that it only imply price of anarchy for independent valuation distributions. 
However, similar analysis framework for correlated distributions holds with the presence of secondary markets. 

\begin{definition}[\citealp{lucier2011gsp,roughgarden2017price}]\label{def:smooth private deviation}
For any $\lambda>0,\mu\geq 1$, auction $\mech$ with action space $\actions$ is $(\lambda,\mu)$-semi-smooth
if for any type profile $\type$,
there exists action distributions $\{\dista_i(\type_i)\}_{i\in [n]}$ such that 
for any action profile $\action\in \actions$, 
\begin{align*}
\sum_{i\in[n]} \expect[\action'_i\sim \dista_i(\type_i)]{\util_i(\mech(\action'_i, \action_{-i});\type_i)} \geq \lambda \wel(\type) - \mu \rev(\action;\mech)
\end{align*}
\end{definition}

\begin{theorem}[\citealp{lucier2011gsp}]\label{thm:smooth imply poa correlate}
Letting $\dists$ be the family of all possible distributions, 
for any $\lambda>0,\mu\geq 1$, if a mechanism $\mech$ is $(\lambda,\mu)$-semi-smooth, 
then for any correlated prior distribution of the types, 
the price of anarchy is at most $\frac{\mu}{\lambda}$,
i.e., $\poa(\mech, \dists) \leq \frac{\mu}{\lambda}$.
\end{theorem}

\begin{theorem}\label{thm:smooth private deviation}
For any mechanism $\mech_1$ which is $(\lambda,\mu)$-semi-smooth,
and any secondary market mechanism $\mech_2$ satisfying voluntary participation and weak budget balance, 
the combined market $\mech_C = (\mech_1, \mech_2)$ is $(\lambda,\mu)$-semi-smooth. 
\end{theorem}
The proof of \Cref{thm:smooth private deviation} is similar to 
\Cref{thm:smooth} and hence the proof is omitted here. 
One observation of our reduction framework is that we do not require refinements on the equilibrium such subgame perfect equilibrium in the combined market to show that the price of anarchy is small. 

\begin{theorem}[\citealp{lucier2011gsp}]
For AdWords auction,
generalized second price auction is $(\sfrac{1}{2}, 2)$-semi-smooth. 
\end{theorem}

\begin{corollary}
For AdWords auction,,
given any secondary market satisfying voluntary participation and weak budget balance,
the price of anarchy of generalized second price auction is at most $4$ when the prior distribution is correlated. 
\end{corollary}

% \bjl{We know that PoA doesn't get worse when adding a secondary market, but does the PoA strictly improve?  If we assume only voluntary participation and weak budget balance then the answer is no; for example, the secondary market could be the trivial one that never allows trade.  But maybe under additional restrictions.  

% More concretely: suppose the secondary market is one where ``sellers'' declare values first, then ``buyers'' do.  That is, everyone first declares values for the items they already own, then they declare their value for additional items.  After all declarations are made, efficient trade occurs at the minimal market-clearing price.  Would PoA strictly improve?}

% \section{Inefficiency of Secondary Market}
% Here we consider a simple example of single item auction with two i.i.d.\ buyers. 
% The valuation distribution $\dist$ of the buyer is uniform in $[0,1]$. 
% For first price auction without secondary market, 
% the unique Bayesian Nash equilibrium is efficient and symmetric.
% Now assume that in the secondary market, 
% the agents can trade at price $\frac{1}{2}$ if and only if 
% one agent winning the item has value at most $\frac{1}{2}$
% and the other agent has value at least $\frac{1}{2}$.
% Next we will show that in the combined market, no equilibrium can guarantee efficient outcome. 

% Suppose by contradiction, there exist efficient Bayesian Nash equilibrium strategy $\sigma$. 
% Since the equilibrium is efficient, 
% and when both agents have value above $\frac{1}{2}$, 
% no trade happens in the secondary market. 
% The equilibrium strategy for agents with value above $\frac{1}{2}$ is strictly monotone and symmetric, 
% except for a set of values with measure 0. 
% Similarly, the equilibrium strategy for agents with value below $\frac{1}{2}$ is also strictly monotone and symmetric, 
% except for a set of values with measure 0. 
% Let $S_1 \subseteq (0, \frac{1}{2}), S_2 \subseteq (\frac{1}{2}, 1)$ 
% be the set of values with measure $\frac{1}{2}$ each
% such that the equilibrium strategy is monotone and symmetric.
% Next we show that 
% $\sup_{v\in S_1} \sigma(v) \leq \inf_{v\in S_2}\sigma(v)$. 

% Again suppose by contradiction that $\sup_{v\in S_1} \sigma(v) > \inf_{v\in S_2}\sigma(v)$. 
% Then there exists $\bar{\delta}, \bar{\epsilon}>0$ such that 
% $\sigma(\frac{1}{2}-\delta) > \sigma(\frac{1}{2}+\epsilon)$
% for any $\delta\in(0, \bar{\delta}), \epsilon\in (0, \bar{\epsilon})$. 
% % Let $b_2$ be the optimal bid of agent with value $$
% To simplify the notation, let 
% $v_1 = \frac{1}{2}+\epsilon, b_1 = \sigma(v_1)$, and 
% $v_2 = \frac{1}{2}-\delta, b_2=\sigma(v_2)$. 
% Let $q(b; \sigma) = \Pr_{\val\sim U[0,1]}[b > \sigma(\val)]$ be the probability the agent wins the item with bid $b$ given equilibrium strategy $\sigma$ for the opponent. 
% Let $p_1(b;\sigma) = \Pr_{\val\sim U[0,1]}[\val < \frac{1}{2} \given b < \sigma(\val)]$
% be the probability the value of the opponent is lower than $\frac{1}{2}$ conditional on losing the item with bid $b$.
% % Note that $p(b;\sigma) = \frac{1}{2q(b; \sigma)}$.
% Similarly define $p_2(b;\sigma) = \Pr_{\val\sim U[0,1]}[\val > \frac{1}{2} \given b > \sigma(\val)]$.
% We omit $\sigma$ in the notations when it is clear from the context. 
% Since $b_2$ is the equilibrium bid for agent with value $\frac{1}{2}-\delta$, 
% we have 
% \begin{align}\label{eq:util opt 2}
% q(b_2)(\frac{p_2(b_2)}{2} + v_2(1-p_2(b_2)) - b_2) 
% \geq q(b_1)(\frac{p_2(b_1)}{2} + v_2(1-p_2(b_1)) - b_1) 
% \end{align}
% Moreover, letting $\delta' > 0$ be a sufficiently small constant, 
% we have 
% \begin{align*}
% &u_1(b_2; v_1) = q(b_2)(v_1 - b_2) + (1-q(b_2))(v_1-\frac{1}{2})p_1(b_2)\\
% &\geq q(b_1)(v_1 - b_1) + (\epsilon+\delta)(q(b_2) - q(b_1))
% + \delta(p_2(b_2) - p_2(b_1)) 
% + (1-q(b_2))(v_1-\frac{1}{2})p_1(b_2)\\
% &= u_1(b_2; v_1)
% % q(b_1)(v_1 - b_1) 
% % + (1-q(b_1))(v_1-\frac{1}{2})p_1(b_1)
% + \epsilon \cdot (p_1(b_2)(1-q(b_2)) - p_1(b_1)(1-q(b_1)))
% + (\epsilon+\delta)(q(b_2) - q(b_1))
% + \delta(p_2(b_2) - p_2(b_1)) \\
% &\geq u_1(b_2; v_1)
% - \epsilon \cdot p_1(b_1)(1-q(b_1))
% + \epsilon\cdot (q(b_2) - q(b_1)) - \delta'\\
% &= u_1(b_2; v_1)
% - \epsilon \cdot \Pr_{\val\sim U[0,1]}[\val < \frac{1}{2} \text{ and } b_1 < \sigma(\val)]
% + \epsilon\cdot \Pr_{\val\sim U[0,1]}[b_1 < \sigma(\val) < b_2]
% (q(b_2) - q(b_1)) - \delta' \\
% &> u_1(b_2; v_1).
% \end{align*}
% The first inequality holds by simply apply inequality \eqref{eq:util opt 2} and rearrange the terms. 
% The second inequality holds for sufficiently small $\delta$. 
% The last inequality holds because 
% there exists a strictly positive measure of agent with value between $(\frac{1}{2}, \frac{1}{2}+\epsilon)$ 
% that will bid between $b_1$ and $b_2$,
% which implies 
% $\Pr_{\val\sim U[0,1]}[b_1 < \sigma(\val) < b_2] > \Pr_{\val\sim U[0,1]}[\val < \frac{1}{2} \text{ and } b_1 < \sigma(\val)]$.
% Note that the above inequality is a contradiction to the assumption that $b_1$ is the equilibrium bid for $v_1$. 

% Note that by the above paragraph, 
% the only possible equilibrium strategy is strictly monotone and symmetric for all values in $[0,1]$ except a zero measure set. 
% In this case, no trade happens in the secondary market, 
% and the agents' utility is the same as if there is no secondary market. 
% Thus, the equilibrium strategy for each agent is $\sigma(\val) = \frac{\val}{2}$ in the auction environment.
% Next we verify that this is not an equilibrium strategy in the combined market by showing that 
% there exists a set of values with positive measure such that the best response is not $\sigma(\val)$ given that the opponent follows this strategy. 
% For $\val \in (0, \frac{1}{2})$, 
% the utility for bidding $\frac{\val}{2}$
% is 
% \begin{align*}
% \val(\val - \frac{\val}{2}) = \frac{\val^2}{2}.
% \end{align*}
% However, the utility for bidding $\frac{1}{3}$
% is 
% \begin{align*}
% \frac{2}{3}(\frac{3}{4}\val + \frac{1}{8}-\frac{1}{3}) 
% = \frac{\val}{2} > \frac{\val^2}{2}.
% \end{align*}
% Thus, we conclude that there does not exist a Bayesian Nash equilibrium that guarantees efficiency.  





\section{Inefficiency with Secondary Markets}
\subsection{Mult-unit Auction with Decreasing Marginals}
In this section, we consider the case when the seller sell $m$ units of identical items to 
$n$ agents with decreasing marginals for each extra unit. 
Here we focus on the uniform price auctions.

\begin{definition}
An agent has \emph{decreasing marginal} valuation if $v_i(j) - v_i(j-1)$ is decreasing for any $j\in [m]$.
\end{definition}
\begin{definition}
The \emph{uniform price auction} asks each agent $i$ to report marginal values $b_{i,1}\geq \cdots\geq b_{i,m}$. 
The items are allocated to the $m$ highest marginal bids and each winning unit is charged with price equals then $(m+1)$th marginal bid.
\end{definition}

\citet{de2013inefficiency} showed that the price of anarchy is at most $3.15$ for uniform price auctions when agents bid at most there marginal values. 
However, we show that uniform price auction is not robust in the presence of the secondary market. 
First note that agents may try to win the item and resell in the secondary market, 
thus it is reasonable that under equilibrium, agents will bid above their marginal valuation for the item. 
Here we consider a specific secondary market,
where each pair of agents $i,i'$ simultaneously make bids for trading the item among them. 
Assuming agent $i$ holds $m_i$ units of the item, for each unit $j\in[m_i]$, if the marginal bid of agent $i'$ for unit $j$ is higher than that for agent $i$, 
unit $j$ is sold to agent $i'$ with price equals the average bid. 
If one agent sells more items than her endowment in the secondary market, 
then the market break ties uniform randomly and let the agent sell until supply lasts.

\begin{example}
There are $3$ agents and $m$ items. 
Agent $1$ has marginal values $0$ for all the units. 
Agent $2$ has marginal values $1$ for all the units. 
Agent $3$ has marginal value $2$ for the first unit and $0$ for the rest units with probability $\frac{m-2}{m-1}$, 
and has marginal values $0$ for all the units with probability $\frac{1}{m-1}$. 
The expected optimal welfare is $m-1+\frac{2(m-2)}{m-1}$. 

Suppose the uniform price auction break ties in the order of $1>2>3$. 
In the first market, agent $1$ bids $1-\frac{1}{m-1}$ for the first $m-2$ units and $0$ for the rest $2$ units. 
Agent $2$ bids $1$ for the first unit and $0$ for the rest units. 
Agent $3$ always truthfully bids her marginal values for the units.
In the secondary market, if agent $1$ has exactly $m-1$ units, 
she offers selling price $1-\frac{1}{m-1}$ to agent $2$ for $m-1$ units, 
agent $2$ offers buying price $1-\frac{1}{m-1}$ to agent $1$ for $m-1$ units, 
and items are traded with price $1-\frac{1}{m-1}$. 
Otherwise, agent $1$ offers selling price $1$ to agent $2$ for all her units, 
agent $2$ offers buying price $0$ to agent $1$, 
and items are not traded.
We can verify that this is an equilibrium for all agents, 
and the expected welfare in equilibrium is $\frac{4m-6}{m-1}$.
Thus the price of anarchy is $\Omega(m)$.
\end{example}


\subsection{Second Price Auction}
The performance of the second price auction depends on the equilibrium refinement we impose on the market. 
When there is no secondary market, 
there exists inefficient equilibrium for the second price auction, 
while under the refinement of undominated strategies, 
all equilibria are efficient. 

When there are secondary markets, 
there exists inefficient equilibrium even under the refinement of undominated strategies.
For simplicity, we focus on two agent setting 
and in the secondary market, the winner in the auction posts a take-or-leave-it offer to the other agent. 

% There are some mechanisms that have small price of anarchy under equilibrium refinements. 
% Here we show that with the presence of the secondary markets,
% price of anarchy may have unbounded increase under the same equilibrium refinement.  
\begin{example}
% For single item auction with two agents, 
% the second price auction $\mech_1$ has price of anarchy $\poa(\mech_1, \dists) = 1$ for any family of distributions $\dists$ under undominated strategies.
% 
% Suppose the secondary market allows the winner to post a price to the other agent. 
Consider the case where agent 1 has value 0 for the item and agent 2 has value distribution $F_1(v) = \frac{v-1}{v}$ for $v\in [1, H]$ and $F_1(H) = 1$. 
In the combined market, agent 1 bids $H$ in the auction and sells the item at price $H$ in the secondary market. 
Agent $2$ bids $0$ in the auction and accepts the offer from agent 1 if the price is weakly lower than the private value. 
This is an equilibrium strategy that survives the refinement of undominated strategies, 
and the price of anarchy is $\log H$, which is unbounded when $H\to\infty$. 
\end{example}

However, if we impose stronger refinement notion of iterative elimination of weakly dominated strategies, 
then second price auction is efficient for all equilibria if the secondary market satisfies ex post individual rational and weak budget balance
and bids are not revealed in the secondary market. 
Moreover, it is sufficient to have two rounds of elimination of weakly dominated strategies.


\begin{theorem}
For single-item setting, given any secondary market satisfying voluntary participation and weak budget balance
where bids are not revealed, 
all equilibria in second price auction are efficient.  
\end{theorem}
\begin{proof}
For any agent~$i$, let $p_i$ be the expected payment to agent $i$ when she resells the item. 
Since the secondary market satisfies voluntary participation,
we have $\val_i\leq p_i$. 
Next we claim that any bid $b_i > p_i$
in the auction environment 
is weakly dominated by bidding $p_i$ in the auction environment and reselling the item with expected payment $p_i$ in the secondary market. 
Note that the only difference for agent $i$
is the case that the highest bid of the opponents in the auction is in $(p_i,b_i)$.
In that case, she strictly benefits from lowering the bid and not winning the item since her value is $\val_i\leq p_i$.

Conditional on the event that for all agents, 
the bids in the auction are weakly lower than their price charged for reselling the item 
in the secondary market, 
it is a weakly dominant strategy for all agents to bid their value in the auction, 
since all agents get weakly higher utility for winning in the auction than in the secondary market. 
Thus the allocation is efficient in the auction, 
and no trade happens in the secondary market. 
All equilibria are efficient in the combined market. 
\end{proof}





\section{Price of Stability}
In this section, we analyze the price of stability result in the combined market. 
First, we made the following assumption on the secondary market $\mech_2$. 

\begin{assumption}\label{asp:opt out}
For any initial allocation $\alloc$, there exists an action profile $\hat{\action}^S\in \actions^S$ such that for any agent $i$, any action $\action^S_i$, we have 
\begin{align*}
u_i(\mech_2(\action^S_i, \hat{\action}^S_{-i}, \alloc); \type_i)
\leq u_i(\mech_2(\hat{\action}^S, \alloc); \type_i)
= u_i(\alloc; \type_i)
\end{align*}
\end{assumption}
This assumptions implies that for all initial allocation $\alloc$ in the secondary market, 
there exists an action profile which is a pure Nash equilibrium. 
This action profile can be viewed as the option that all agents choose to opt out the secondary market. 
A simple example of the secondary market that satisfies \Cref{asp:opt out} is the single item environment where $\mech_2$ asks agents 
to simultaneously place bids for the item, and trade with the price offered by the agent holding the item
to a random agent with bid higher than the price.
The action profile where the agent holding the item bids infinity and all other agents bid $0$ satisfies \Cref{asp:opt out} for this particular mechanism $\mech_2$.
Next we define 
\begin{align*}
\pos(\mech, \dists) = \max_{\dist\in \dists} 
\frac{\wel(\dist)}{\max_{\strategy\in \SPE(\dist, \mech)}\{\wel(\mech, \strategy, \dist)\}}
\end{align*}
as the price of stability of mechanism $\mech$ within the family of distributions $\dists$,
where $\SPE$ degenerate to $\BNE$ when $\mech$ is a normal-form game. 

\begin{theorem}\label{thm:pos}
For any mechanism $\mech_C = (\mech_1, \mech_2)$
with $\mech_2$ satisfying \Cref{asp:opt out},
for any family of distributions $\dists$,
we have 
\begin{align*}
\pos(\mech_C, \dists) \leq \pos(\mech_1, \dists). 
\end{align*}
\end{theorem}
\begin{proof}
For any allocation $\alloc$, let $\hat{\action}^S_{\alloc}$ be the action profile that satisfies \Cref{asp:opt out} in secondary market. 
For any distribution $\dist\in \dists$ strategy $\strategy^F\in \BNE(\dist, \mech_1)$, 
let $\strategy^S$ be the strategy that always chooses action profile $\hat{\action}^S_{\alloc}$ for all types given that the initial allocation in the secondary market is $\alloc$. 
It is easy to verify that there is no deviating strategy for any player $i$ in any subgame. 
Therefore, $\strategy^C = \strategy^F\times\strategy^S \in \SPE(\dist,\mech_C)$, 
and the expected welfare given strategy $\strategy^C$ in combined market $\mech_C$
equals the expected welfare given strategy $\strategy^F$ in first market $\mech_1$.
\end{proof}

\section{Efficiency in Symmetric Environments}

% \mbc{seems to me that this entire paragraph should be erased as a better motivation is presented in the second paragraph:}
% In \citet{garratt2006speculation}, 
% the authors showed that the efficiency guarantee of the first price auction is not robust 
% in the presence of secondary market 
% if there is a speculator. 
% In their model, they assume that the speculator has public valuation $0$ for the item. 
% In this section, we will show that speculation does not deteriorate the efficiency guarantee for first price auction
% if the valuation distribution of all buyers (including the speculator) are symmetric, 
% and this result is robust to any form of the secondary market, including asymmetric secondary markets. 
% % \mbc{Maybe we should remark that for IID bidders there is a unique NE in FPA that is monotone and thus efficient, so the PoS of any combined market running FPA and then an some mechanism $M_2$ that is weakly BB and IR is 1. This is so as the original NE is still NE with no trade in the secondary market. \\ Was the IID setting studied? Are there asymmetric equilibria? }

In this section, 
we consider the setting of a seller that has a single item for sale, and two buyers with i.i.d.\ valuation distributions. 
In \citet{hafalir2008asymmetric}, 
the authors consider the same setting for a specific family of secondary markets
and show that for first price auction, 
the equilibrium in the combined market is efficient 
if (1) no information on valuations and bids is  revealed in the secondary market,
and (2) the bids in the auction are non-decreasing. 
We generalize their result by showing the efficiency result for any secondary market satisfying 
ex post individual rationality and ex post weak budget balance.\footnote{This is a stronger requirement than individual rationality and weak budget balance. However, this is sufficient to capture natural secondary markets such as winner in the auction posting price to other players in the secondary markets.}
% We assume that the seller adopts the first price auction 
% and has no control over the secondary market. 
% Here, we still make the assumption the  
Moreover, we have weaker assumption on the information revealed in the secondary market. 
In this section, we assume that (1) valuations of the agents are not directly revealed in the secondary market\mbe{, yet bids can be revealed (either only one, or both)},
and (2) the bids in the auction are non-decreasing. 
The techniques used in this section is similar to \citet{chawla2013auctions}, 
where the authors showed that the the unique equilibrium for first-price auction is efficient for symmetric distribution
if there is no secondary market. 

% An additional assumption for the result in this section is that no information about the private valuation of the buyer is revealed in the secondary market. 

% \begin{assumption}\label{asp:no value reveal}
% For any agent $i$, any valuation $\val_i, \val'_i$
% and any action $\action_i$, 
% if agent $i$ chooses action $\action_i$ when her value is 
% $\val_i$ or $\val'_i$, 
% then neither the mechanism nor the other buyer can distinguish between $\val_i$ and $\val'_i$. \mbc{Is there a reason to talk about abstract "actions" instead of simply bids in the FPA?}
% \end{assumption}
\begin{assumption}\label{asp:no value reveal}
The valuations of all agents are not directly revealed in 
the secondary market.
\mbc{I suggest replacing this by: No information but potentially (some of the) bids is revealed after the first market. In particular, the valuations of all agents are  never directly revealed.}
\end{assumption}

% \mbc{It is not clear what is the assumption - is this an assumption about information that is disclosed after the FPA ? How is it different than  assuming that only FPA bids are revealed? }

In comparison to \citet{hafalir2008asymmetric}, 
our assumption is weaker since we allow the bids of the agents to be revealed, 
and let agents to update their belief about others' valuation based on the bid profiles. 
The importance of \Cref{asp:no value reveal} is to establish the payment identity in the combined market. 

\begin{lemma}\label{lem:payment identity}
% \mbc{I would make the "any combined market" more explicit. Also, we should probably explicitly refer to assumption 8 (is it the same as revealing nothing but bids? If so maybe say this explicitly): "Consider combining FPA with any $M_2$ that is IR and weak BB such that the combined market satisfies assumption 8. Letting..." }
For any combined market satisfying \Cref{asp:no value reveal}, i.e., the valuations of the agents are not directly revealed in the secondary market, 
letting $\alloc$ and $\pay$ be the interim allocation of the agents, 
then for any agent $i$, 
we have 
\begin{align*}
\pay_i(\val_i) = \val_i\alloc_i(\val_i) - \int_0^{\val} \alloc(z) \dd z + \pay_i(0).
\end{align*}
\end{lemma}
The proof of \Cref{lem:payment identity} follows directly from  \citet{myerson1981optimal}, 
thus omitted here. 

\begin{theorem}\label{thm:symmetric efficiency}
For single-item setting with two i.i.d.\ buyers,
% that have} 
% monotone submodular valuations,
given any secondary market satisfying ex post individual rationality, ex post weak budget balance, and \Cref{asp:no value reveal},
all Nash equilibria are efficient, 
i.e., the price of anarchy is $1$, 
for first-price auction and all-pay auction
if the valuation distribution is continuous in bounded intervals
and the bids in the auction environment are non-decreasing in values.
\end{theorem}
In \Cref{thm:symmetric efficiency}, we obtain efficiency for both first price auction 
and all-pay auction.
The proof for those auctions are similar and in the following parts, we only show it for the first price auction. 
Moreover, in the statement of the theorem, we make the assumption of non-decreasing bids. 
We conjecture that this assumption is not necessary for the efficiency results. 
\begin{figure}[t]
\centering
\input{fig/symmetric}
\vspace{-6pt}
\caption{\label{f:symmetric dist}
Asymmetric bid functions $\bid_1$ and $\bid_2$. 
}
\end{figure}
\begin{proof}[Proof of \Cref{thm:symmetric efficiency}]
Since the secondary market satisfies ex post individual rationality and ex post weak budget balance, 
for any valuation profile such that the allocation in the auction environment is efficient, 
no trade occurs in the secondary market, 
and hence the allocation is efficient in the combined market.
If both agents use the same strictly increasing strategy, 
the allocation is efficient in the auction environment for all valuation profiles, 
and hence it is efficient in the combined market. 
Moreover, if both agents use the same monotone strategy while there exists an interval $(\val',\val'')$ such that the bids are the same for values in this interval,
any agent with value in the interval can strictly increase her bid by an infinitesimal amount to strictly increase her utility, 
contradicting to the assumption that the strategies are sustained under equilibrium.

We next assume that strategies of the two agents are monotone yet asymmetric.
For any value $\val^*$ such that $\bid_1(\val^*) > \bid_2(\val^*)$,
let $\bar{\val}\leq \val^*$ be the infimum value such that $\bid_1(\bar{\val}) \geq \bid_2(\bar{\val})$, 
and $\bar{\val}'\geq \val^*$ be the supremum value such that $\bid_1(\bar{\val}') \geq \bid_2(\bar{\val}')$. 
This is illustrated in \Cref{f:symmetric dist}.
% First we show that $\util_1(\bar{\val}) = \util_2(\bar{\val})$
% and $\util_1(\bar{\val}') = \util_2(\bar{\val}')$. 

First we show that $\util_1(\bar{\val}) = \util_2(\bar{\val})$. 
The claim that $\util_1(\bar{\val}') = \util_2(\bar{\val}')$ holds similarly. 
We claim that $\lim_{\val\to\bar{\val}} \bid_1(\val) = \lim_{\val\to\bar{\val}}\bid_2(\val)$. 
Suppose in contradiction that 
$\lim_{\val\to\bar{\val}} \bid_1(\val) > \lim_{\val\to\bar{\val}}\bid_2(\val)$
and let $\epsilon = \lim_{\val\to\bar{\val}} \bid_1(\val) - \lim_{\val\to\bar{\val}}\bid_2(\val)$. 
Note that by assumption $\epsilon>0$.
There exists $\val \in (\bar{\val}-\frac{\epsilon}{4}, \bar{\val})$
such that $\bid_1(\val) \in (\lim_{\val\to\bar{\val}}\bid_2(\val) + \frac{\epsilon}{2}, \bid_2(\bar{\val}))$ \mbc{why?}.
Thus agent 1 with value $\val$ can lower her bid by $\frac{\epsilon}{2}$ without affecting the allocation in the auction 
with utility increase $\frac{\epsilon}{2}$ when she wins the item. 
Moreover, since the secondary market is ex post individually rational and ex post weak budget balance, 
when she wins the item in the auction, 
the utility for reselling the item in the secondary market is at most $\frac{\epsilon}{4}$. 
Hence it is strictly beneficial for her to deviate her bid, 
a contradiction that $\bid_1, \bid_2$ are equilibrium strategies. 
Therefore, we must have $\lim_{\val\to\bar{\val}} \bid_1(\val) = \lim_{\val\to\bar{\val}}\bid_2(\val)$, 
and we define the limit as $\bid^*$. 
For any $\delta > 0$, 
let $\delta' \in (0, \delta)$ be the constant such that $\bid_1(\val), \bid_2(\val) \in (b^*-\delta, b^*)$ for any $\val \in (\bar{\val}-\delta',\bar{\val})$.
The utility of agent 1 with any value $\val \in (\bar{\val}-\delta', \bar{\val})$ is 
\begin{align*}
\util_1(\val) \geq (\val - b^*) \cdot \Pr_{\val\sim\dist_2}[\val \leq \bar{\val}]
\geq (\bar{\val} - b_2(\val)) \cdot \Pr_{\val\sim\dist_1}[\val \leq \bar{\val}] - 2\delta
\geq \util_2(\bar{\val}) - 2\delta.
\end{align*}
The first inequality holds because player 1 can always choose to bid $b^*$ in the auction
and retain the same utility in the combined market since the secondary market is individual rational. 
The last inequality holds since agent 2 can only resell the item to agent 1 with payment below $\bar{\val}$ since 
the secondary market is ex post individual rational
and under equilibrium bid $\bid_2(\val)$, 
she only wins the item if her opponent's value is below $\bar{\val}$. 
Similarly we can have 
$\util_2(\bar{\val}) \geq \util_1(\bar{\val}) - 2\delta$
for any $\val \in (\bar{\val}-\delta', \bar{\val})$
and hence $\lim_{\val\to\bar{\val}} \util_1(\val) = \lim_{\val\to\bar{\val}}\util_2(\val)$.
Since the interim utility is a continuous function of the valuation, we have
$\util_1(\bar{\val}) = \util_2(\bar{\val})$.

% Both $\bar{\val}$ and $\bar{\val}'$ are finite and well defined since the support of the valuation distribution is bounded. 


%If the FPA is not efficient, then
% Assume that there exists $\bar{\val} < \bar{\val}'$
% such that $\bid_1(\bar{\val}) = \bid_2(\bar{\val})$, 
% $\bid_1(\bar{\val}') = \bid_2(\bar{\val}')$,
% and $\bid_1(\val) > \bid_2(\val)$ for any $\val\in (\bar{\val},\bar{\val}')$. 
% % \mbc{will it always exist? what if not?}
% We will show that in this case, the only possible scenario for the asymmetry in the bid functions is that 
% agents will re-trade in the secondary market such that the allocation is efficient. 
% Note that other cases such as bids $\bid_1(\val) > \bid_2(\val)$ for any $\val$ can be proved similarly. 
% Thus the proof for those special cases is omitted here 
% and the readers can refer to \citet{chawla2013auctions} for a detailed discussion. 

% First we show that $\util_1(\bar{\val}) = \util_2(\bar{\val})$
% and $\util_1(\bar{\val}') = \util_2(\bar{\val}')$. 
% This is due to the format of the first price auction. 
% Note that for each agent $i$, if $\val_i = \bar{\val}$, 
% then agent $i$ wins the item if and only if 
% her bid is higher than her opponent.
% Since $\bid_1(\bar{\val}) = \bid_2(\bar{\val})$
% and bids are monotone, 
% this is equivalent to the situation that
% her value is higher than her opponent.\footnote{This trivially holds if the bids functions are strictly increasing at $\bar{\val}$. 
% If there is an interval of valuations $[\val_1,\val_2]$ with the same bids $\bid_1(\bar{\val})$, 
% we can simply consider }
% Since the allocation is efficient in this case, 
% no trade happens in the secondary market (due to ex post individual rational and ex post budget balance). 
% Thus, we have 
% \begin{align*}
% \util_1(\bar{\val}) = (\bar{\val} - \bid_1(\bar{\val})) \cdot \Pr_{\val\sim\dist_2}[\val \leq \bar{\val}]
% = (\bar{\val} - \bid_2(\bar{\val})) \cdot \Pr_{\val\sim\dist_1}[\val \leq \bar{\val}]
% = \util_2(\bar{\val}).
% \end{align*}
% Similarly we also have $\util_1(\bar{\val}') = \util_2(\bar{\val}')$.
Moreover, by \Cref{lem:payment identity}, 
we have that 
\begin{align*}
\int_{\bar{\val}}^{\bar{\val}'} \alloc_1(\val) \dd \val
= \int_{\bar{\val}}^{\bar{\val}'} \alloc_2(\val) \dd \val.
\end{align*}
Since the secondary market satisfies ex post individual rational and ex post weak budget balance, 
no trade happens in the secondary market if agent $i$ wins the item and $\val_i > \val_{-i}$.
Thus, $\alloc_1(\val) \geq \alloc_2(\val)$ since $\bid_1(\val) > \bid_2(\val)$ for any $\val\in (\bar{\val},\bar{\val}')$.
In order for the integral of allocations to coincide, 
we have $\alloc_1(\val) = \alloc_2(\val)$ for any $\val\in (\bar{\val},\bar{\val}')$, 
which implies that 
the item is sold from agent $i$ to $-i$ in the secondary market 
if agent $i$ wins the item and $\val_i < \val_{-i}$.
Therefore, the allocation in the combined market is efficient.
\end{proof}




\section{Price of Anarchy for Revenue}
In \citet{hartline2014price}, the author showed that 
when there is no secondary markets, 
first price auction or all-pay auction with monopoly reserve
guarantees constant approximation to the optimal revenue. 
However, their technique does not extend to the setting 
when there are secondary markets.
The main reason is that their analysis requires agents with value below the monopoly reserve will not win the item, 
which is not guaranteed in our setting since agents may win the item in the secondary market even if their value is below the reserve price in the auction. 
\citet{carroll2019robustly} characterized the optimal mechanism that are robust to the format of the secondary market. 
The authors only considered the revenue under the best equilibrium, 
and the revenue guarantee under worst equilibrium is left as an open problem. 
In this section, we show that for any valuation distribution,
there exists a simple mechanism that guarantees constant approximation to the optimal revenue 
given any secondary market under worst equilibrium. 

\begin{theorem}\label{thm:anonymous reserve}
For first price auction or second price auction with anonymous reserve, 
if the bids of the buyers are not revealed in the secondary market
and the secondary market satisfies weak budget balance and voluntary participation, 
then the item is sold if there exists an agent with value strictly above the reserve price. 
\end{theorem}
\begin{proof}
Given anonymous reserve price $r$,
if for all agents, the bid of the agents is weakly above $r$
when their value is strictly above $r$, 
then \Cref{thm:anonymous reserve} holds. 

Now suppose there exists an agent $i$ with value $\val_i > r$
such that the bid of agent $i$ is $b_i < r$. 
Next we consider three different cases for the bid of other agents. 
\begin{enumerate}
\item Suppose $\max_{j\neq i} b_j < r$. In this case, the item is not sold to any agent, 
which implies that agent $i$ strictly benefits from deviating to bid $r$ and win the item with price $r$
since $b_i - r > 0$. 

\item Consider the case where $\max_{j\neq i} b_j \geq r$ and the item is sold to agent $j^*\neq i$ even if agent $i$ has bid $r$. 
For agent $i$, by deviating the bid to $r$, 
the allocation of the auction is not affected and 
since the bids are not revealed in the secondary market, 
the utility of agent $i$ remains the same.

\item Consider the case where $\max_{j\neq i} b_j = r$ and when agent $i$ deviate the bid to $r$, she wins the item.
Since the mechanism is individual rational, 
the price paid to agent $j^*$ for reselling the item in the secondary market is at least $r$, 
which implies that the utility of agent $i$ in the combined market is at most $\val_i - r$. 
Moreover, by bidding $r$ and winning the item, 
the utility of agent $i$ is at least $\val_i - r$. 
\end{enumerate}
By combining those situations, for agent $i$, 
the utility for bidding at least $r$ is weakly higher than the utility for bidding strictly below $r$. 
Moreover, the equality holds only when the item is sold to another agent $j^*$ with probability 1 when agent $i$ bids strictly below $r$. 
This implies that the item is always sold when there exists an agent with value strictly above~$r$. 
\end{proof}

Note that in \Cref{thm:anonymous reserve}, it is crucial to assume that the bids are not revealed in the secondary market. 
It is reasonable to assume that the mechanism designer has control over bid information and chooses not the reveal such information to the secondary market. 
The following example illustrate the failure of \Cref{thm:anonymous reserve} if bids are revealed. 
\begin{example}
Consider there are $3$ agents. 
Agent $1$ has value $1.1$, agent $2$ has value $0$ or $2$ with probability $\frac{1}{2}$ each, 
and agent $3$ has value $0$ or $5$ with probability $\frac{1}{2}$ each. 
Suppose the auctioneer chooses second price auction with reserve price $1$. 
Now consider the secondary market where if agent $1$ bids at least $1$, then no trade can ever occur. 
If agent $1$ bids below $1$, 
then agent $2$ has the option to sell the item to agent $3$, 
where agent $2$ receive price $2$ for the sale 
and agent $3$ pays price $3$ for the item. 
Agent $1$ receives price $1$ if the trade happens. 
It is easy to verify that in this setting, 
the following is an equilibrium strategy for all agents. 
Agent $1$ bids $0$, 
agent $2$ bids $5$ if her value is $5$ and $0$ otherwise, 
and agent $3$ bids $1$ if her value is $2$ and $0$ otherwise.
Moreover, under this equilibrium, the item is not sold if both agent $2$ and agent $2$ has value $0$, 
and the revenue of the mechanism is only $\frac{3}{4}$
even though agent $1$ has value strictly above reserve price $1$ with probability $1$. 
\end{example}

By \Cref{thm:anonymous reserve}, we can show that 
if the bids are not revealed in the secondary market, 
the revenue of first price auction or second price auction with anonymous reserve $r$ given any secondary market and equilibrium strategy 
is at least the revenue of posting the 
%same reserve 
price of $r$ 
to all agents when there are no secondary markets. 
In \citet{jin2019tight}, the authors showed that when there are no secondary markets, 
if the valuation distributions are regular, 
anonymous pricing is a $2.62$-approximation to the optimal revenue. 
Combining the results, we obtain the following corollary for price of anarchy on revenue. 
% Let $\rev(\dist)$ be the optimal Bayesian revenue 
% when the valuation distribution is $\dist$
% and there is no secondary markets. 
% Let 
% \begin{align*}
% \poar(\mech, \dists) = \max_{\dist\in \dists} 
% \frac{\rev(\dist)}{\min_{\strategy\in \BNE(\dist, \mech)}\{\rev(\mech, \strategy, \dist)\}}
% \end{align*}
% be the price of anarchy for revenue given mechanism $\mech$ and the family of distributions $\dists$.

\begin{corollary}\label{cor:poa revenue}
When the valuation distributions are regular for all agents
and when mechanism $\mech_1$ is first price auction or second price auction with optimally chosen anonymous reserve, 
the price of anarchy for revenue given the combined market 
$\mech_C = \mech_1\times\mech_2$
is at most 2.62, 
if the bids of the buyers are not revealed in the secondary market
and the secondary market $\mech_2$ satisfies weak budget balance and voluntary participation. 
\end{corollary}

% Note that in the definition of the price of anarchy for revenue, 
% we only compare to the benchmark of optimal Bayesian revenue 
% when there is no secondary markets. 
% One interpretation for this benchmark is that it can be viewed as an upper bound on the max-min revenue of the seller, 
% where the maximum is taken over the auction mechanism, 
% and the minimum is taken over the secondary market
% and the equilibrium selection. 
% Another reason for this choice is that the optimal revenue with secondary markets might be too large to approximate 
% if the valuation of the agents are revealed in the secondary markets, 
% which is illustrated in the following example. 
Finally, next example provides justifications for only comparing to the optimal revenue without secondary market
in the definition of price of anarchy for revenue. 
\begin{example}\label{exp:large rev}
Suppose there are two agents. Agent 1 has value 1 and agent 2 has valuation distribution $F(\val) = 1-\frac{1}{\val}$ for any $\val \in [1,H)$ and $F(H)=1$. 
The optimal revenue for the combined market is $\log H$ 
if the secondary market satisfies that the valuations are public information and agent 1 has full bargaining power.
This is obtained by selling the item to agent 1 with price $\log H$, 
and agent 1 resales the item to agent 2 with price $\val$.
In contrast, for any auction mechanism, the worst case revenue over the all possible secondary markets 
is at most the optimal revenue when is no secondary markets, 
which is at most 1. 
The gap is unbounded when $H\to \infty$.
\end{example}





\section{Efficiency for Single Strategic Agent}
In this section, we consider the special case of selling a divisible item to a group of agents where there is only a single strategic agent. 
We assume that all other agents are price taker and the demand of those agents are infinitesimal. 
The strategic agent is ignorant of the individual valuation function of other agents but aware of the aggregated valuation function. 
The benefit of studying this model is to characterize the behavior of the agent in the combined market without worrying about the equilibrium selection in the secondary market. 
Let $v_1(q)$ be the value of the strategic agent for quantity $q$ 
and $v_2(q)$ be the aggregated welfare of the rest of the agents.
\begin{definition}
An agent $i$ has \emph{monotone and decreasing marginal valuation} if 
$v'_i(q) \geq 0, v''_i(q) \leq 0$ for any $q\in [0, 1]$. 
\end{definition}
% We assume that all agents have monotone and decreasing marginal valuation, 
% which implies that $v'_1(q) > 0, v''_1(q) < 0$ and $v'_2(q) > 0, v''_2(q) < 0$.
% We show that under this assumption, 
% the welfare in the combined market is always weakly higher than the welfare without secondary market. 
In the auction environment, all agents simultaneously declare valuation functions. 
% and the item is sold at the market clearing price \mbc{there might be more than one clearing price. need to break ties carefully}. 
In the secondary market, 
the strategic agent offers a uniform trading price 
to the price takers, 
and those agents purchase the item from the strategic agent if the marginal value for the additional item exceeds the price, 
and sell the item if the marginal value for the item is below the price. 
% In the secondary market, 
% the strategic agent offers a uniform price to the price takers and purchase \mbc{the fact he buys from them and never sells to them is a result, not an assumption. We need to allow both options apriori} from all other agents the fraction of their allocations with marginal value below the price. 


\begin{definition}
Let $A$ and $B$ be two subsets of $\reals$. 
We say that $B$ is weakly greater than $A$ according to the strong set order (denoted by $B \geq A$) if for any $a \in A$ and $b \in B$, if $a > b$, then
$a \in B$ and $b \in A$.
\end{definition}

% \mbc{The theorem below seems to be missing the solution concept. 
% Here we need to add something like "In the next theorem the "social welfare of a market"
% is the set of all possible welfare values obtained when considering all subgame perfect equilibria of that market." (and maybe also discuss undominated strategies - I think they might not be needed here.)}

\begin{theorem}\label{thm:strong set order}
If all agents have monotone and decreasing marginal valuations, 
when the price-takers bid truthfully 
and the strategic agent best responses, 
the social welfare in the combined market is weakly greater than the welfare without secondary market in strong set order.
\end{theorem}
\begin{proof}
First note that if the strategic agent 
enters the secondary market with endowment $q_0$,
% acquired $q_0$ fraction of the item in the auction, 
% in the secondary market, 
his utility in the secondary market 
is $u_1(q, q_0)=v_1(q)-v'_2(1-q)(q-q_0)$
if he receives a total of $q$ fraction of the items when he posts price $p = v'_2(1-q)$. 
Thus the optimal price $p^*$ in the secondary market satisfies
\begin{enumerate}
    \item $v'_2(1-q^*) = p^*$;
    \item $q^* = \argmax_q u_1(q, q_0)$.
\end{enumerate}
Since the utility function $u_1(q, q_0)$ is supermodular in $q$ and $q_0$. 
Note that the optimal choice $q^*$ may not be unique. 
By Topkis's Theorem, 
$q^*(q_0)$ is monotone increasing in $q_0$ in strong set order. 
Moreover, if $q_0 = 0$, the resulting allocation $q^*(0)$ is equivalent to the allocation of all agents participate the auction without secondary market. 
Thus in the combined market, for the optimal strategy of the strategic player, 
his allocation is greater than the case without secondary market in strong set order. 
Moreover, the marginal value of the strategic agent for quantities between $q^*(q_0)$ and $q^*(0)$ is higher than the rest of the agents. 
Hence the social welfare only improves in strong set order. 
\end{proof}

A corollary to \Cref{thm:strong set order} is that,
if the optimal choice of the strategic agent is unique in the auction without secondary market, 
then the optimal welfare weakly improves with the presence of secondary market. 
% \mbc{I am not able to follow this remark, please clarify.}

\mbc{as discussed, it might be good to add an example in which the welfare is strictly larger and the drawing with the intuition of the proof (in the spirit of what Brendan drew)}

==> content/outline.tex <==

\subsection{New Outline}

Pitch for applied modeling track paper, where we claim to model carbon markets.

\begin{enumerate}
    \item Intro: carbon markets; impact of speculation; informal secondary markets not under designer's control.
    \item Model -- general, then examples of carbon license instantiations.  Remove the "acquiring more information" material.  Focus on multi-unit setting.  Rewrite to be focused on the carbon market setting in the language.  (I.e., not just "a seller").  Connect with examples of particular auction forms used in practice, and also examples of secondary markets.  Compare with carbon tax, grandfathered allocation.
    \begin{enumerate}
        \item Extension 1: speculators can be better informed.
        \item Extension 2: combinatorial setting.
    \end{enumerate}
    \item Section 3: bad examples for auctions, what goes wrong.  Discussion: acting as monopolist; demand reduction; implicit complementarities; etc.
    \item Section 4: Positive result / reduction.  Implication for multiunit auctions (discriminatory price auction is robust)
    \item Section 5: Posted pricing (prior-dependent).  Use prophet inequalities, but median-based doesn't work necessarily.  Show that 1/2 mean does work.\mbc{how do we plan to fit posted price in the general story? Currently there are periodic auction, and these posted price are more like "online" decision making.  }  \yl{Intro suggests that people have rejected discriminatory auction due to the concern of paying too high a price (the so-called winner’s curse) for lack of information on market price. I think the posted pricing mechanism will not have this concern as the prices are transparent, which could be a motivation for posted price.}
\end{enumerate}


==> content/refine.tex <==
\section{Equilibrium Refinements}
\label{sec:refine}
Since $\mechc$ proceeds in multiple rounds, it will be helpful to consider notions of equilibrium that ensure that strategies are rational in each round.  We will use the notion of 
%
%In proving our negative results, we not only prove them for BNE, but rather for 
sequential equilibrium (SE), a refinement of BNE proposed in \citet{kreps1982sequential}.\footnote{One can view Sequential Equilibrium as a notion of subgame perfection tailored to settings of incomplete information.}
A fully general definition of SE is beyond the scope of this paper; the following description is semi-formal.  Roughly speaking, in an SE of our game each agent maintains beliefs about how other agents will act in each round, updates those beliefs using Bayes' rule in response to information given between the auction and the secondary market, and in each round every agent acts in a utility-maximizing way given their beliefs.  An important subtlety is how Bayes' rule should be applied to events with $0$ probability, such as under deviations from the equilibrium.  This is handled by thinking of each strategy as a limit of `trembling' strategies in which all possible actions have a positive chance of being observed.

%Roughly speaking, in an SE of our game each agent's behavior in the second round is a best response to a rational set of beliefs about what others will do in the second round, given all information revealed in the first round.  An important subtlety is how beliefs are defined under deviations from the equilibrium; this is handled by thinking of each strategy as a limit of `totally-mixing' strategies in which all possible actions have a positive chance of being observed.
%This comes to illustrate that the negative results are not derived by strange ``non-credible" strategies. 
More formally, a strategy profile $\sigma$ is a \emph{sequential equilibrium} if there exists a belief assessment\footnote{A belief assessment is a mapping from a history of observations to a belief (distribution) over the actions of others.} $\beta$ such that 
\begin{enumerate}
\item For every agent and given any history of observations, following the strategy $\sigma$ is a best response to the belief specified by~$\beta$; and
\item there exists a sequence of totally mixing strategy profiles $\{\sigma^k\}_{k\geq 1}$ converging to $\sigma$ 
and a sequence of beliefs $\{\beta^k\}_{k\geq 1}$ converging to $\beta$ such that $\beta^k$ is consistent with each agent applying Bayes' rule to all observations, under the assumption that agents are applying strategy profile $\sigma^k$.
\end{enumerate}
Every SE is a BNE, but the reverse is not always true.  All of our positive results will hold for all BNE (even those that are not SE), and all of our negative results will apply even when restricting to SE.

We first show that the strategy profile constructed in \Cref{exp:spa} are sequential equilibrium, 
and undominated (survives a single round of  elimination of weakly dominated strategies). 

\begin{lemma}\label{lem:SPA-example-undominated}
	The strategies presented in \Cref{exp:spa} are undominated. Additionally, they form a sequential equilibrium. 
\end{lemma}
\begin{proof}
We first show that this is indeed an equilibrium in undominated strategies.  
The strategy $\sigma_1$ of agent $1$ is to bid $H$ in the auction and if she wins, post the utility maximizing price of $H$
%\footnote{\mbc{Note that it is easy to slightly modify the valuation distribution $F_2$ to make price $H$ the unique profit maximizing price, so this result does not hinge on ties and how they are broken.\yl{Since player 1 has value 1 for the item. Thus in the example H is already the unique profit maximizing price.}}}
 to agent $2$.\footnote{Note that her utility from price $p\in [1,H]$ is $p\cdot \frac{1}{p} + 1\cdot (1-\frac{1}{p}) =2-\frac{1}{p}$, which is maximized at $p=H$. } 
 We claim there is no other strategy of agent $1$ that dominates this one. 
Consider any other strategy $\sigma_1'$ of agent $1$: 
agent $1$ submits a randomized bid $b_1$ sampled from a bid distribution $F_1$ in the auction,
and if she wins, she offers the item at price $q_1$ to agent $2$. Note that as bidders get no signal after the auction, $q_1$ cannot depend on the bid of agent $2$.
To prove that $\sigma_1$ is undominated, we claim that $\sigma_1$ is strictly better than $\sigma_1'$ when agent 2 plays the following strategy: 
(1) places deterministic bid $b' < H$ in the auction such that $b_1< b'$ with positive probability measure;\footnote{If $b_1=H$ for sure, then clearly $\sigma_1$ is strictly better than $\sigma_1'\neq \sigma_1$ since for such $\sigma_1'$ it must hold that $q_2\neq H$,  but $H$ is the unique optimal offer.}
(2) resells the item with price $H$ conditional on winning; 
and (3) purchases the item if the price is no more than $H$ conditional on losing. 
Note that the utility of agent 1 is the same under $\sigma_1'$ and $\sigma_1$ if the realized bid $\bid_1 \geq b'$, 
and the utility of agent 1 is strictly smaller under $\sigma_1'$ if the realized bid $\bid_1 < b'$. 

{Similarly, the strategy $\sigma_2$ of agent $2$ is to bid $0$ in the auction and accept the price from agent $1$ if and only if the price is at most her value. Consider any other strategy $\sigma_2'$ of agent $2$: 	agent $2$ submits a randomized bid $b_2$ sampled from a bid distribution $F_2$ in the auction,	and if she wins, she offers the item at price $q_2$ to agent $1$.
Consider the following strategy of agent 1: 
(1) places deterministic bid $b' > 0$ in the auction such that $b_2 > b'$ with positive probability measure;
(2) resells the item with price $0$ conditional on winning; 
and (3) does not purchase the item in secondary market conditional on losing.
Note that the utility of agent 2 is the same under $\sigma_1'$ and $\sigma_1$ if the realized bid $\bid_2 \leq b'$, 
and the utility of agent 2 is strictly smaller under $\sigma_1'$ if the realized bid $\bid_2 > b'$.}

We next show that this strategy profile is indeed a sequential  equilibrium.  
{First note that for all agents, conditional on losing in the auction, 
it is dominant strategy to accept the price if and only if the price is below her value.  So this price-taking behavior is always sequentially rational regardless of beliefs.
Conditional on winning, agent 2 has no uncertainty about the type of agent 1 and would never sell the item.  If agent 1 wins, then the rational belief of agent $1$ about agent $2$'s valuation in the secondary market is identical to the prior. 
Under this belief, posting price $H$ conditional on winning is the dominant strategy for agent~1. 
Moreover, this belief is consistent with the equilibrium strategy of the agents, 
i.e., there exists a sequence of totally mixing strategy $\strategy^k$ where in the auction,
agent $1$ bids $H$ with probability $1-\frac{1}{k}$ and bids uniformly in $[0,H]$ with probability $\frac{1}{k}$, 
and agent $2$ bids $0$ with probability $1-\frac{1}{k}$ and bids uniformly in $[0,H]$ with probability $\frac{1}{k}$ regardless her valuation. 
Note that $\strategy^k \to \strategy$, and the strategy $\strategy^k$ reveals no information of agent's value for any $k$. 
Thus $\beta^k$ is identical to the belief $\beta$ that the agent has under equilibrium for all $k$. 
}
\end{proof}



%In \Cref{exp:spa}, we have illustrated that 
Thus, \Cref{exp:spa} shows that the  second-price auction is not robust (in the sense of low PoA) to the introduction of a secondary market, 
%in the combined market
even under the refinement of undominated strategies (and of sequential equilibrium). 
In the next theorem, 
we show that under the stronger refinement of two round elimination of weakly dominated strategies (TWDS), all equilibria of the combined market are efficient, if we combine the second-price auction 
with  the specific secondary market where the winner in the auction posts a price to other agents, and no information is released from the auction.\footnote{This is the same secondary market we considered in \Cref{exp:spa}.} 
% \bjl{This is for a specific secondary market format.  We should make this clear, or prove a more general theorem.}
%\yl{This result only holds for specific posted pricing as secondary market.
%This is the same secondary market we consider in \Cref{exp:spa}. }
\begin{theorem}\label{thm:refine spa}
Consider the single-item setting with buyers with independently drawn valuations. % , each from a regular distribution.
Fix the auction $\mechf$ to be the second-price auction, 
and $\mechs$ to be a price posting mechanism.\footnote{Here the winner in the auction posts a price $p$ to other agents in the secondary market, 
and the item is traded at price $p$ if there is at least one other agent willing to accept the price. 
Ties are broken arbitrarily. } 
%and fix any trade mechanism $\mechs$. %secondary market $\mechs$ satisfying voluntary participation and weak budget balance. 
Consider the combined market 
$\combinedGameNoSignal$
in which bidders get no signal after the auction. % in which not information is revealed after the auction.
Then under the refinement of two-round elimination of weakly dominated strategies, 
all Bayesian Nash equilibria in the combined market are efficient.
%OLD: 
%For single-item setting, if the winner posts a take-or-leave-it offer to the other agent in the secondary market  and no information is revealed in the secondary market, under the refinement of two-round elimination of weakly dominated strategies,  all Bayesian Nash equilibria in the combined market for the second price auction are efficient.
  
\end{theorem}
\begin{proof}
%\bjl{Rephrased the proof to make it clear we're fixing an equilibrium then arguing about its properties.  Double-check this is correct!}
Fix any equilibrium of the combined mechanism that survives iterated elimination of weakly dominated strategies.  (We will later show that such an equilibrium is guaranteed to exist.)  For any agent~$i$, let $p_i$ be the price agent $i$ charges when she resells the item under this equilibrium.  
%\bjl{Couldn't the price posted depend on the bid agent $i$ placed in round $1$?  Since agent $i$ learns something from the fact that they won with that bid, so their posterior over the other agent's value changes.}
Since agent $i$ also maximizes her utility in the secondary market,
we have $\val_i\leq p_i$. 
Next we claim that any bid $b_i > p_i$
in the first stage
would be weakly dominated by bidding $p_i$ 
and reselling the item with price $p_i$ in the secondary market. 
Since no information is revealed in the secondary market,
the only difference for agent $i$
is the case that the highest bid of the opponents in the auction is in the range of $(p_i,b_i)$.
In that case, she strictly benefits from lowering the bid and not winning the item since her value is $\val_i\leq p_i$.  We can therefore assume that $b_i \leq p_i$ for each agent $i$ with probability $1$.

Conditional on the event that for all agents, 
the bids in the auction are weakly lower than their price charged for reselling the item 
in the secondary market, 
it is a weakly dominant strategy for all agents to bid their value in the auction, 
since all agents get weakly higher utility for winning in the auction than in the secondary market. 
Finally, given that all agents are not underbidding in the auction, 
the allocation is efficient under any Nash equilibrium
since if there exists any agent that overbids,
in order for this to sustain under equilibrium, 
anytime the allocation is inefficient in the auction, 
the winner in auction, denoted by $i$, must have bids $b_i > v_i$, 
and her utility is strictly less than bidding $v_i$ unless 
she resales the item to the highest other bidder $i'$ with price $b_{i'} = \val_{i'}$.
This is efficient since all agents with bid below $b_{i'}$ must also have value below $\val_{i'}$ since none of agents are underbidding.
%Thus the allocation is efficient in the auction, 
%and no trade happens in the secondary market. 
%All equilibria are efficient in the combined market. 
\end{proof}


The next example illustrates that the idea of two-rounds of elimination of weakly dominated strategies generates efficiency outcomes 
does not generalize beyond the single-item auctions. 
%in settings other than single item auction, the price of anarchy can be large even under the strong refinement of 
%iterative elimination of weakly dominated strategies. 
More specifically, we consider the multi-unit auction 
for agents with decreasing marginal valuations. 
%Here we focus on the uniform price auctions.
%
%\mbc{this definition now appears in the model - remove? }
%% \begin{definition}
%% An agent has \emph{decreasing marginal} valuation if $v_i(j) - v_i(j-1)$ is decreasing for any $j\in [m]$.
%% \end{definition}
%\begin{definition}
%	For the multi-unit auctions setting with non-increasing marginal valuations, the \emph{uniform price auction} asks each agent $i$ to report marginal values $b_{i,1}\geq \cdots\geq b_{i,m}$. 
%The items are allocated to the $m$ highest marginal bids and each winning unit is charged with price equals the $(m+1)$th marginal bid.
%\end{definition}
For uniform-price auctions, \citet{de2013inefficiency} showed that the price of anarchy is at most $3.15$ when agents bid at most their marginal values. 
Moreover, overbidding is weakly dominated when there is no secondary market. 
However, those results does not extend in the presence of the secondary market. 
In the combined market, agents may try to win the item and resell in the secondary market, 
and thus it is reasonable that under equilibrium, agents will bid in the auction above their marginal valuation for the item.
In the following, we first provide a formal definition for the multi-unit setting and the mechanisms we interested in. 

\medskip\noindent\textbf{Multi-unit Settings.}
%In the \emph{multi-unit} setting, 
The seller has $m$ identical indivisible items to sell to $n$ agents,
and the feasibility constraint is $\feasibles = \{(\alloc_i)_{i\in[n]}: \alloc_i\in \{0,\dots,m\}, \forall i\in [n] \text{ and } \sum_i\alloc_i \leq m\}$.  One might restrict to \emph{non-increasing marginal valuations}, in which for any type $\type_i\in \types_i$ it holds that 
$\val_i(j; \type_i)- \val_i(j-1; \type_i)$ is non-negative and (weakly) decreasing in $j$, for $j\in [m]$. 
A valuation is \emph{sub-additive} if $\val_i(j; \type_i)+ \val_i(j'; \type_i) \geq \val_i(j+j'; \type_i)$ for any $j,j'\in[m]$ such that $j+j'\leq m$.

\medskip\noindent\textbf{Mechanisms. }
Each agent $i$ simultaneously submit a bid $(a_{i1},\dots,a_{im})\in A_i= \reals_{\geq 0}^{m}$ representing her $m$ marginal values, with $a_{i1}\geq \dots \geq a_{im}$.
Then $m$ units of items are greedily allocated to the bidders of the $m$ highest marginal bids. Payments are set as follows: 
	\begin{itemize}
	\item
	\emph{discriminatory auction}: 
	Agent $i$ winning $x_i$ units of items pays her highest $x_i$ marginal values  $\sum_{j=1}^{x_i} a_{ij}$.
	\item \emph{uniform-price auction} 	Agent $i$ winning $x_i$ units of items pays for each unit  
	the $(m+1)$-th highest marginal bid within the $n\times m$ reported marginals. 
	\end{itemize}

Note that the discriminatory auction is a generalization of the first-price auction in the multi-unit setting
and the uniform-price auction is a generalization of the second-price auction in the multi-unit setting. 
In the following example, we consider a uniform-price auction followed by a
%the 
secondary market where the agents that win items in the auction can sequentially post prices to other agents as a take-or-leave-it offer. 
The equilibrium constructed in the following example illustrate the failure of extending the approach in \cref{thm:refine spa} to multi-unit auctions.
%\yl{I removed the claim about iterative elimination of dominated strategies. Instead I added discussion at the end on why we think uniform-price auction in multi-unit setting could be qualitatively different from second price auction in single item setting.}

\begin{example}\label{exp:uniform price incomplete}
There are two agents and $m$ units of items in the market. 
\begin{itemize}
\item Agent $1$ has value $1$ for each of the $m$ units. 
\item Agent $2$ has value $m$ for the first unit, 
and value $\val$ per unit for each of the other $m-1$ units, 
where the cumulative distribution for value $\val$ is $F(\val) = 1-\frac{1}{\val}$ for $\val \in [1, m)$
and $F(\val) = 1$ for $\val \geq m$. 
\end{itemize}
% Next we show that 
The following profile of strategies is a sequential equilibrium: % for all agents. 
\begin{itemize}
\item Agent $1$ bids $m$ for the first $m-1$ units, and $0$ for the last unit.
Agent $2$ bids $m$ for the first unit, and bids $0$ for the rest of the units.
\item In the secondary market, agent $1$ post price $m$ to agent $2$ for each of the $m-1$ units.
\end{itemize}
It is easy to see that agent $1$ wins $m-1$ units and agent $2$ wins $1$ unit in the auction, and each pays zero. 
The units won by agent $1$ is resold to agent $2$ if and only if the value of the additional units for agent $2$ is $m$, which occurs with probability $\frac{1}{m}$.
One can easily verify this strategy profile is indeed a sequential equilibrium.\footnote{This is because in the secondary market, 
agent $2$ are adopting dominant strategy of accepting the prices if and only if the value is at least the price, 
and agent $1$ is posting the unique utility maximization price given her belief about agent $2$.}
The optimal welfare is $\Theta(m\log m)$ by allocating all items to agent $2$, 
while the expected welfare under the constructed sequential equilibrium is $\Theta(m)$. 
Thus the price of anarchy is $\Omega(\log m)$.
\end{example}

%\paragraph{Proof of undominated strategies}
%\yl{We claim that the following set of strategies survives iterative elimination of weakly dominated strategies. 
%Also it is easy to verify that the set of strategies contains the equilibrium strategies $(\sigma^*_1, \sigma^*_2)$ in \cref{exp:uniform price incomplete}.
%The set of equilibrium strategies $\Sigma_1$ for agent $1$ is to bid $m$ for the first $m-1$ units, and $b\in[0,m)$ for the last unit. 
%Agent $1$ resells the item at price $m$ in the secondary market. 
%The set of equilibrium strategies $\Sigma_2$ for agent $2$ is to bid $m$ for the first units. 
%For value $m$, agent $2$ bids $b\in[0,m)$ for the second unit, 
%and $0$ for the rest units. 
%For value $v<m$, agent $2$ bids $0$ for the last $m-1$ units.
%For all values agent $2$ accepts the price if it is below her marginal value. 
%
%For each strategy of agent $1$ in $\Sigma_1$, suppose there is another strategy 
%
%For each strategy of agent $2$ in $\sigma_2\in \Sigma_2$, for any another strategy $\strategy'_2$, 
%if $\strategy'_2$ bids strictly higher than $0$ for the last $m-1$ units, 
%the utility strictly decreases when agent $1$ chooses strategy $\sigma^*_1$. 
%}


\textbf{Remark:}
In contrast to the case of second-price auction for the  single-item setting, in uniform-price auction for the multi-unit setting there exist strict incentives for the agents to shade bids in the auction (in \cref{exp:uniform price incomplete}, 
the utility of agent $2$ strictly decreases if she increases her bids in the auction), so such underbidding is not dominated, 
even if the price posted by the opponent in the secondary market is at least her bid in the auction.
However, as illustrated in \cref{thm:refine spa}, 
with two rounds of elimination of weakly dominated strategies, 
underbidding in the auction is weakly dominated. 
Moreover, knowing that opponents will shade their bids in the auction while also willing to accept higher prices in the secondary markets, 
agents with low values also have incentives to overbid and win the item for resale. 

%\mbc{should we say few words about us leaving open the possibility that the stronger refinement of  
%	 iterative elimination of dominated strategies can solve the problem? We may also say that we suspect it does not.  }
%	 \yl{My conjecture is that the equilibrium in above example survives the stronger refinement of iterative elimination of dominated strategies. 
%To prove this, we need to find a fixed point of set of strategy profiles that contains the constructed equilibrium strategies, 
%which currently we do not know how to do this formally since considering the strategies on path and off path could be complicated in this setting. }

% Here we consider a specific secondary market,
% where each pair of agents $i,i'$ simultaneously make bids for trading the item among them. 
% Assuming agent $i$ holds $m_i$ units of the item, for each unit $j\in[m_i]$, if the marginal bid of agent $i'$ for unit $j$ is higher than that for agent $i$, 
% unit $j$ is sold to agent $i'$ with price equals the average bids of agent $i$ and $i'$. 
% Moreover, no agent can sell more items than her endowment in the secondary market.


% \begin{example}
% There are $3$ agents and $m$ items. 
% Agent $1$ has marginal values $0$ for all the units. 
% Agent $2$ has marginal values $1$ for all the units. 
% Agent $3$ has marginal value $2$ for the first unit and $0$ for the rest units with probability $\frac{m-2}{m-1}$, 
% and has marginal values $0$ for all the units with probability $\frac{1}{m-1}$. 
% The expected optimal welfare is $m-1+\frac{2(m-2)}{m-1}$. 

% Suppose the uniform price auction break ties in the order of $1>2>3$. 
% In the first market, agent $1$ bids $1-\frac{1}{m-1}$ for the first $m-2$ units and $0$ for the rest $2$ units. 
% Agent $2$ bids $1$ for the first unit and $0$ for the rest units. 
% Agent $3$ always truthfully bids her marginal values for the units.
% In the secondary market, if agent $1$ has exactly $m-1$ units, 
% she offers selling price $1-\frac{1}{m-1}$ to agent $2$ for $m-1$ units, 
% agent $2$ offers buying price $1-\frac{1}{m-1}$ to agent $1$ for $m-1$ units, 
% and items are traded with price $1-\frac{1}{m-1}$. 
% Otherwise, agent $1$ offers selling price $1$ to agent $2$ for all her units, 
% agent $2$ offers buying price $0$ to agent $1$, 
% and items are not traded.
% We can verify that this is an equilibrium for all agents, 
% and the expected welfare in equilibrium is $\frac{4m-6}{m-1}$.
% Thus the price of anarchy is $\Omega(m)$.
% \end{example}

% Note that the equilibrium strategy constructed above survives the refinement of 
% both sequential equilibrium and 
% iterative elimination of weakly dominated strategies. 
The example above illustrates that for multi-unit uniform-price auction, 
even though it is smooth under undominated strategies when there is no secondary markets \citep[c.f.][]{de2013inefficiency}, 
the combined market may have large  price of anarchy not only for BNE but also for sequential equilibria as well as for undominated strategies.
This is in sharp contrast to the discriminatory auction which is smooth without further assumptions \citep[c.f.][]{de2013inefficiency}, 
and in \Cref{thm:poa combined market} we show that the price of anarchy 
for smooth auction is small in the combined market for 
all Bayesian Nash equilibria, even without any refinement. 


==> content/smooth.tex <==
\section{Smooth Framework: Beyond a Single Market}
\label{sec:smooth}
If the agents that are playing in the auction do not take into account the existence of the secondary market and play as if it does not exist,
then clearly any secondary market satisfying weak budget balance and voluntary participation can only increases the expected welfare of the market.
However, rational agents that are aware of the secondary market will take it into account when playing in the auction, and,
%if the allocation is endogenous,  i.e., if the format of the secondary market and agents behavior in it may distort their incentives in participating the auction,
as illustrated in \citet{hafalir2009revenue,garratt2006speculation},
the expected equilibrium welfare may decrease in the combined market due to speculation. 

Explicitly characterizing the associated welfare loss is a laborious task: it requires one to construct and analyze the equilbrium which can depend on the agents' distributions in subtle ways.  This task is complicated even for relatively simple distributions.  \citet{hafalir2009revenue} manage to construct an example with welfare loss of $\frac{2e}{2e-1}$ by studying a single-item 2-agent setting with carefully-chosen type distributions $F_1(v) = (\frac{v}{w})^a$ for $v\in [0,w]$ and $F_2(v) = v^a$ for $v\in [0,1]$ (for given constants $a>0, w>1$).  Their example operates in a very simple economic environment -- a first price auction followed by a posted price secondary market.  Only by transitioning to an i.i.d.\ setting and imposing additional constraints on the mechanism are they able to obtain an efficiency result.  

One might conclude that proving non-trivial upper bounds on the efficiency loss in general settings is intractable.
\iffalse
%We illustrate this with the following example:
\begin{example}[\citealp{hafalir2009revenue}]
\label{example:FPA-welfare-loss}
There is a single item and two agents with valuations drawn independently as follows.
Let $a>0, w>1$ be two constant specified later.
The valuation distribution for agent 1 is $F(v) = (\frac{v}{w})^a$ for $v\in [0,w]$
and the valuation distribution for agent 2 is $F(v) = v^a$ for $v\in [0,1]$.
The item is sold in a first-price auction.
The welfare of the unique equilibrium of the first-price auction (without a secondary market) tends to $\frac{a}{a+1}$ as $w\to\infty$.

Consider the secondary market where the winner can post a deterministic price to the other agent based on her updated posterior belief (after winning with her bid).
There exists an equilibrium in the combined market such that the equilibrium welfare is
$\frac{a}{a+1}\left(1-\frac{(a+1)^{-(a+1)/a}}{a+2}\right)$
when $w\to\infty$.
Thus when $a\to 0$ and $w\to\infty$,
the combined market equilibrium welfare might be smaller than the %\mbc{unique?}\yl{Not proved in literature} auction
equilibrium welfare of the first-price auction by a multiplicative factor of
\begin{align*}
\lim_{a\to 0} \left(1-\frac{(a+1)^{-(a+1)/a}}{a+2}\right)^{-1} = \frac{2e}{2e-1}.
\end{align*}
%\mbc{add an example with FPA in which the introduction of a secondary market reduces equilibrium welfare (ideally for all equilibria, and if not possible, at least for one). The example should later move to the intro and only be referred to here. The secondary market should be ex-post IR and ex-post BB (ideally with 2 independent but not iid agents, so we can contrast it with the iid case). }
\end{example}
%\mbc{Is there a simpler "trivial" example that only shows that there is some loss when adding secondary market? While this example is good for large ratio, such a simpler example might be better for the introduction }\yl{Probability this is the simplest we can find, since people only have explicit equilibrium construction for some special cases of distributions.} \bjl{The example from Section 3.3 might do well as an introductory example.  It shows non-triviality, is significantly simpler, and still illustrates the point about speculation.}\mbc{indeed, but it is a negative example, so we will not be able to say we have a PoA bound for it. }
Thus even for first-price auctions (FPA), there might be a non-negligible welfare loss due to the introduction of a secondary market.
\fi
However, in this section we show that while adding a secondary market might harm welfare, the welfare loss for smooth auctions (such as FPA) can be upper bounded.
The worst-case welfare guarantees of several classical mechanisms (e.g., single-item first-price auction) will not decrease in the combined market, as long as the auction mechanism satisfies certain smoothness properties.  In other words, while the equilibrium welfare may decrease in particular market instances, worst-case guarantees due to smoothness are retained.

%\bjl{Should the following paragraph move to the introduction?  Not sure it fits here.} \mbc{I agree.}
%In \citet{roughgarden2012price, syrgkanis2013composable}, the authors developed the smoothness framework for analyzing the price of anarchy for auction environments, and show that price of anarchy proofs that are based on smoothness imply some very attractive properties. For example, the  extension theorems show that PoA bounds proven using the smooth argument hold not only at Nash equilibrium, but also at no-regret outcomes (\citet{roughgarden2012price} \mbc{expand and make precise. Also, is this the right citation?}).
%In this section, we add another property to the extraordinary list of attractive properties of smooth auctions,
%showing that the smoothness property is preserved for the combined market
%if the secondary market satisfying voluntary participation and weak budget balance.
%Thus our paper highlight another aspect in which smooth auctions are robust - adding an arbitrary secondary market (only satisfying the most fundamental properties of voluntary participation and weak budget balance) does not harm the smoothness of the auction at all.
%As the combined market is smooth, it also inherit all the previously known properties implied by smoothness.

% \yl{removed title for subsection}

%\subsection{Main Results: Smoothness Preservation}\label{sec:smooth-main}
We next prove our main result regarding smoothness preservation: when combining a smooth auction with a secondary market satisfying voluntary participation and weak budget balance, the combined market is smooth with exactly the same parameters.



%Next we illustrate how to generalizes the property of  $(\lambda,\mu)$-smooth to combined markets.
Our main result shows that if an auction is $(\lambda,\mu)$-smooth and we add a secondary market the satisfies voluntary participation and weak budget balance, then the combined market is  $(\lambda,\mu)$-smooth  as well.
One immediate implication of this result  together with \Cref{thm:smooth imply poa} is a PoA bound for product type distributions.

% \begin{theorem}\label{thm:smooth}
% % Fix any secondary market mechanism $\mechs$ satisfying voluntary participation and weak budget balance,  and any signaling protocol $\Gamma$.
% %For any $(\lambda,\mu)$-smooth mechanism $\mechf$,
% If a mechanism $\mechf$ is $(\lambda,\mu)$-smooth for some for $\lambda>0$ and $ \mu\geq 1$,
% then
% for any signaling protocol $\Gamma$ and any trade mechanism $\mechs$,
% the combined market $\combinedGame$ %$\mechc = (\mechf, \mechs)$
%  is $(\lambda,\mu)$-smooth.
% % MB: I have combined the POA implication into the main theorem:
%  Thus,  the price of anarchy of $\mechc$ within the family of all product distributions $\dists^{\Pi}$  is at most $\frac{\mu}{\lambda}$,
%  i.e., $\poa(\mechc, \dists^{\Pi}) \leq \frac{\mu}{\lambda}$.
% \end{theorem}
% \begin{proof}
% Let $\asetfirst, \asetsecond$ be the action space of mechanisms $\mechf, \mechs$ respective,
% and $\asetcombined$ be the action space of the combined market.
% Note that $\acombined\in\asetcombined$ is an extensive form action,
% which is choosing action $\afirst\in\asetfirst$ in the first market,
% and then choosing action $\asecond\in\asetsecond$ based on the allocation, payment, and signal realized in the first market.
% %and $\asetcombined = \asetfirst \times \asetsecond$ be the action space of the combined market.
% For each agent $i$, by voluntary participation,
% there exists action $\hat{a}\second_i \in \asetsecond_i$
% such that her payoff is at least her value of the initial allocation in the secondary market.
% Since mechanism $\mechf$ is $(\lambda,\mu)$-smooth,
% for any type profile $\type$,
% there exists action distributions $\{\dista\first_i(\type)\}_{i\in [n]}$ such that
% for any action profile $\afirst\in \asetfirst$,
% \begin{align*}
% \sum_{i\in[n]} \expect[\hat{\action}\first_i\sim \dista^1_i(\type)]{\util_i(\mechf(\hat{\action}\first_i, \afirst_{-i});\type_i)}
% \geq \lambda \wel(\type) - \mu \rev(\afirst;\mechf).
% \end{align*}
% For any type profile $\type$, let $\{\dista\combined_i(\type)\}_{i\in [n]}$ be the distributions over actions $\hat{\action}\combined_i$ for each agent $i$
% where $\hat{\action}\combined_i$ chooses action $\hat{\action}\first_i$ according to distribution $\dista\first_i(\type)$,
% and chooses action $\hat{\action}\second_i$ regardless of the signal realization $S_i$, or the allocation and payment in the first market.
% %$(\afirst_i, \hat{\action}\second_i)$ for each agent $i$
% %where $\afirst_i \sim \dista\first_i(\type)$.
% For any $\acombined \in \actions\combined$,
% we have
% \begin{align*}
% &\sum_{i\in[n]} \expect[\hat{\action}\combined_i\sim \dista\combined_i(\type)]{\util_i(\mechc(\hat{\action}\combined_i, \acombined_{-i});\type_i)}
% \geq \sum_{i\in[n]} \expect[\hat{\action}\first_i\sim \dista^1_i(\type)]{\util_i(\mechf(\hat{\action}\first_i, \afirst_{-i});\type_i)} \\
% &\geq \lambda \wel(\type) - \mu \rev(\afirst;\mechf)
% \geq \lambda \wel(\type) - \mu \rev(\acombined;\mechc)
% \end{align*}
% where the first inequality holds by the definition of $\hat{\action}^2_i$, the second as  $\mechf$ is $(\lambda,\mu)$-smooth,
% and the last inequality holds since mechanism $\mechs$ is weakly budget balanced.
% \end{proof}

Note that \Cref{thm:smooth} does not depend on the details of the mechanism in the secondary market
or the information released in the secondary market.
%or the utility function of the agents. \bjl{The comment about utility functions is a bit confusing. I'm tempted to remove that part or reword.  E.g., the result imposes no additional restrictions on valuation functions.}
Moreover, our reduction framework does not require refinements on the equilibrium such as sequential equilibrium in the combined market to show that the price of anarchy is small.

%\bjl{Added the following paragraph of discussion about the significance of this applying to BNE.}MB: good.

This latter point about sequential equilibrium deserves some additional discussion. % As we have shown in \Cref{example:FPA-welfare-loss}, 
Note that speculation behavior can lead to a loss of welfare at equilibrium even when all participants apply sequentially rational strategies.
%That is, even if agents cannot commit at the time of the auction to behave irrationally in the secondary market by, e.g., making threats of mutually detrimental retaliation.
\Cref{thm:smooth} bounds this loss by showing that the smoothness of an auction mechanism extends to the game with a secondary market.  Moreover, this result holds even for equilibria that are not sequentially rational.  In other words, \Cref{thm:smooth} applies even for Bayes-Nash equilibria in which agents can commit to (possibly irrational) behaviors in the secondary market off the equilibrium path, such as mutually detrimental retaliation.\footnote{For example, one bidder might commit to not offering an item in the secondary market (even if she believes a beneficial trade is possible) if a competing bidder bids more than some threshold in the auction.  Such a threat is not sequentially rational, and is therefore excluded in a sequential equilibrium.  But there may be a Bayes-Nash equilibrium in which the competitor responds to the threat by reducing their auction bid as demanded.  Note that the threat is never actually executed on the equilibrium path in this hypothetical example, so it is detrimental to welfare only indirectly through the change of behavior it induces.  An implication of \Cref{thm:smooth} is that the welfare impact of such threats cannot be too large when the auction is smooth.}  Of course, since all sequential equilibria (or perfect Bayesian equilibria) are Bayes-Nash equilibria, \Cref{thm:smooth} implies a welfare guarantee for all such sequentially rational equilibria as well.  For further discussion of the issue of equilibrium refinements, including refinements beyond sequential rationality, see \Cref{sec:refine}.

%\bjl{I suspect we'll want more discussion about how subgame perfection (doesn't) enter here.  I.e., pointing out that our resulting PoA bounds will therefore also hold for all subgame perfect equilibria, as this refinement only removes equilibria.}

%\mbc{Seems like our result says that smoothness does not degrade even if we add a third market (and fourth and so on) when agents are aware of these markets. Should we remark about this?} \bjl{Added a brief remark.} \mbc{I was thinking more in the direction of saying that after we combined a smooth auction with a trade mechanism we get a new smooth mechanism, which we can not view as a smooth auction. Maybe an advantage here is that it is clear we have signaling in each step (while combining with trade mechanisms it might not be that explicit)   }

We also note that \Cref{thm:smooth} extends directly to settings with multiple secondary markets executed sequentially, with information released between each market.
This is because combining a smooth auction with a trade mechanism results with a new smooth mechanism (with the same parameters), which we can now view as a smooth auction to be combined with the next trade mechanism.
%This is because any sequence of trade mechanisms executed one after the other could be modeled as a single (more complex) trade mechanism.

From \Cref{thm:smooth} and prior smooth auction results from the literature we state the following corollary which formally restates the results summarized in \Cref{table:smooth}:


%Combining \Cref{thm:smooth} and  \Cref{thm:smooth imply poa} we derive as an immediate corollary our main result regarding independent prior distributions. The smoothness for auctions in the first market is derived in the literature,  which is summarized in \Cref{tb:smooth}.
%\bjl{The following statement seems redundant, since it subsumes \Cref{thm:smooth}.  I recommend just stating \Cref{thm:smooth}, then moving directly to corollaries where we list the PoA implications.} \yl{substitueted the theorem with the following corollary}
%\begin{theorem}\label{thm:smooth imply poa combined}
%%Fix any secondary market mechanism $\mechs$ satisfying voluntary participation and weak budget balance, and any signaling protocol $\Gamma$.
%If a mechanism $\mechf$ is $(\lambda,\mu)$-smooth for some for $\lambda>0$ and $ \mu\geq 1$,
%then
%for any signaling protocol $\Gamma$ and any trade mechanism $\mechs$,
%the combined market $\combinedGame$
% is $(\lambda,\mu)$-smooth.
%Moreover,
%% for any independent prior distribution of the types $F\in \dists^{\Pi}$,
%the price of anarchy of $\mechc$ within the family of all product distributions $\dists^{\Pi}$  is at most $\frac{\mu}{\lambda}$,
%%for any independent prior distribution of the types, the price of anarchy is at most $\frac{\mu}{\lambda}$,
%i.e., $\poa(\mechc, \dists^{\Pi}) \leq \frac{\mu}{\lambda}$.
%\end{theorem}

\begin{corollary}\label{cor:poa combined}
Consider settings with independent prior distributions.
Consider any trade mechanism $\mechs$, any signaling protocol $\Gamma$
and the combined market $\combinedGame$.
\begin{itemize}
%\item For single-item setting, if $\mechf$ is the first-price auction, then the combined market $\mechc$ is $(1-\sfrac{1}{e}, 1)$-smooth and it has price of anarchy at most $\sfrac{e}{(e-1)}$.

\item
% \mbc{an alternative version of the above, consider  adding the citations to all others like this:}
For single-item setting, if $\mechf$ is the first-price auction, as it is  $(1-\sfrac{1}{e}, 1)$-smooth \citep{roughgarden2012price}, then the combined market $\mechc$
is $(1-\sfrac{1}{e}, 1)$-smooth and it has price of anarchy at most $\sfrac{e}{(e-1)}$.

%\cite{roughgarden2012price}
% \cite{syrgkanis2013composable}
% \cite{de2013inefficiency}

\item
For single-item setting, if $\mechf$ is the all-pay auction,
 as it is  $(\sfrac{1}{2}, 1)$-smooth \citep{roughgarden2012price},
then the combined market $\mechc$
is $(\sfrac{1}{2}, 1)$-smooth and it has price of anarchy at most $2$.

\item
For multi-unit setting with decreasing marginal valuations,
if $\mechf$ is the discriminatory auction,
as it is  $(1-\sfrac{1}{e}, 1)$-smooth \citep{de2013inefficiency},
then the combined market $\mechc$
is $(1-\sfrac{1}{e}, 1)$-smooth and it has price of anarchy at most $\sfrac{e}{(e-1)}$.

\item
For multi-unit auctions with subadditive valuations,
if $\mechf$ is the discriminatory auction,
as it is  $(\sfrac{1}{2}-\sfrac{1}{2e}, 1)$-smooth \citep{de2013inefficiency},
then the combined market $\mechc$
is $(\sfrac{1}{2}-\sfrac{1}{2e}, 1)$-smooth and it has price of anarchy at most $\sfrac{2e}{(e-1)}$.

\item
For combinatorial auctions with submodular valuations,
if $\mechf$ is the simultaneous first-price auction,
as it is  $(1-\sfrac{1}{e}, 1)$-smooth \citep{syrgkanis2013composable},
then the combined market $\mechc$
is $(1-\sfrac{1}{e}, 1)$-smooth and it has price of anarchy at most $\sfrac{e}{(e-1)}$.

\item
For combinatorial auctions with submodular valuations,
if $\mechf$ is the simultaneous all-pay auction,
as it is   $(\sfrac{1}{2}, 1)$-smooth \citep{syrgkanis2013composable},
then the combined market $\mechc$
is $(\sfrac{1}{2}, 1)$-smooth and it has price of anarchy at most $2$.

\end{itemize}
\end{corollary}


%Thus, for product distributions, we have proven a robust welfare guarantee for the combined market generated by
%any $(\lambda,\mu)$-smooth mechanism and any secondary markets satisfying voluntary participation and weak budget balance.
%As \Cref{thm:smooth imply poa} is proven only for independent value distributions, \Cref{thm:smooth} likewise applies only to product distributions.
%As it turns out, we can derive similar results for correlated distributions based on semi-smoothness \citep{lucier2011gsp}.
%
%
%%One limitation for \Cref{thm:smooth} and above applications for $(\lambda,\mu)$-smoothness is that it only implies price of anarchy for independent valuation distributions. However, similar analysis framework for correlated distributions also holds with the presence of secondary markets.
%
%\begin{definition}[\citealp{lucier2011gsp,roughgarden2017price}]\label{def:smooth private deviation}
%Auction $\mech$ with action space $\actions$ is \emph{$(\lambda,\mu)$-semi-smooth} for $\lambda>0$ and $\mu\geq 1$,
%if for any type profile $\type$,
%there exists action distributions $\{\dista_i(\type_i)\}_{i\in [n]}$ such that
%for any action profile $\action\in \actions$,
%\begin{align*}
%\sum_{i\in[n]} \expect[\action'_i\sim \dista_i(\type_i)]{\util_i(\mech(\action'_i, \action_{-i});\type_i)} \geq \lambda \wel(\type) - \mu \rev(\action;\mech)
%\end{align*}
%\end{definition}
%
%The main difference between the definition of semi-smooth and smooth is that the deviating action distribution $\{\dista_i(\type_i)\}_{i\in [n]}$ in semi-smooth only depends on the private type $\theta_i$ of~$i$,
%and not entire the type profile $\theta$.
%
%\begin{proposition}[\citealp{lucier2011gsp}]\label{thm:semi-smooth imply poa}
%% Let $\dists$ be the family of all possible distributions.
%If a mechanism $\mech$ is $(\lambda,\mu)$-semi-smooth for $\lambda>0$ and $\mu\geq 1$,
%then % for any correlated prior distribution of the types $F\in \dists$,
%the price of anarchy of $\mech$ within the family of all distributions $\dists$
%is at most $\frac{\mu}{\lambda}$,
%i.e., $\poa(\mech, \dists) \leq \frac{\mu}{\lambda}$.
%\end{proposition}
%
%Similarly to \Cref{thm:smooth}, we next shows that combining a $(\lambda,\mu)$-semi-smooth auction with any signaling protocol and any trade mechanism results with a combined market that is $(\lambda,\mu)$-semi-smooth.
%One immediate implication of this result  together with \Cref{thm:semi-smooth imply poa} is a PoA bound for arbitrary (non necessarily product)  distributions.
%
%
%\begin{theorem}\label{thm:smooth private deviation}
%	If a mechanism $\mechf$ is $(\lambda,\mu)$-semi-smooth for some for $\lambda>0$ and $ \mu\geq 1$,
%	then
%	for any signaling protocol $\Gamma$ and any trade mechanism $\mechs$,
%	the combined market $\combinedGame$ %$\mechc = (\mechf, \mechs)$
%	is $(\lambda,\mu)$-semi-smooth.
%	Thus, the price of anarchy of $\mechc$ within the family of all  distributions $\dists$  is at most $\frac{\mu}{\lambda}$,
%	i.e., $\poa(\mechc, \dists) \leq \frac{\mu}{\lambda}$.	
%% OLD version:	
%%Fix any secondary market mechanism $\mechs$ satisfying voluntary participation and weak budget balance, and any signaling protocol $\Gamma$. For any mechanism $\mechf$ which is $(\lambda,\mu)$-semi-smooth, the combined market $\combinedGame$ % $\mechc = (\mechf, \mechs)$ is $(\lambda,\mu)$-semi-smooth.
%\end{theorem}
%The proof of \Cref{thm:smooth private deviation} is essentially identical to
%\Cref{thm:smooth} (up to replacing $\dista_i(\type)$ by  $\dista_i(\type_i)$) and hence omitted here. %\mbc{as the proof is short and as we only have one short proof in this section, I suggest we do add the proof for \cref{thm:smooth private deviation}. }\yl{I think since the proof is identical, there is no need for repeating the arguments.}\bjl{I also prefer not to repeat the identical proof.} MB: If identical, I am ok omitting.
%
%We can now use results regarding semi-smooth auction from the literature to prove that the corresponding combined markets are semi-smooth.
%\begin{proposition}[\citealp{roughgarden2017price}]\label{prop:semi-smooth first}
%For the single-item setting with any prior distribution, the first-price auction is $(1-\sfrac{1}{e}, 1)$-semi-smooth.
%\end{proposition}
%
%Combining \Cref{prop:semi-smooth first,thm:smooth private deviation}, we derive as an immediate corollary for price of anarchy for combining first-price auction with any trade mechanism,  for  all prior distributions.
%\begin{corollary}\label{cor:FPA-cor}
%Consider the single-item setting with any prior joint distribution (possible correlated).
%If $\mechf$ is the first-price auction then for  any signaling protocol $\Gamma$ and any trade mechanism $\mechs$,
%the combined market $\combinedGame$ is
%$(1-\sfrac{1}{e}, 1)$-semi-smooth, and it has price of anarchy at most $\sfrac{e}{(e-1)}$.
%\end{corollary}
%\yl{removed the entire subsection for refinement. Should we add a sentence here reference to \cref{sec:refine}?}\mbc{yes}


%\yl{remove below as well?}
%Combining \Cref{thm:semi-smooth imply poa} and  \Cref{thm:smooth private deviation} we derive as an immediate corollary our main result regarding all prior distributions:
%\begin{theorem}\label{thm:semi-smooth imply poa combined}
%	If a mechanism $\mechf$ is $(\lambda,\mu)$-semi-smooth for some for $\lambda>0$ and $ \mu\geq 1$,	then 	for any signaling protocol $\Gamma$ and any trade mechanism $\mechs$, 	the combined market $\combinedGame$ %%$\mechc = (\mechf, \mechs)$
%	is $(\lambda,\mu)$-semi-smooth.
%	Moreover,  	the price of anarchy of $\mechc$ within the family of all  distributions $\dists$  is at most $\frac{\mu}{\lambda}$, 	i.e., $\poa(\mechc, \dists) \leq \frac{\mu}{\lambda}$.
%% OLD: 	Fix any secondary market mechanism $\mechs$ satisfying voluntary participation and weak budget balance. If a mechanism $\mechf$ is $(\lambda,\mu)$-semi-smooth for some for $\lambda>0$ and $ \mu\geq 1$, then the combined market $\mechc = (\mechf, \mechs)$ is $(\lambda,\mu)$-semi-smooth, and moreover,   the price of anarchy of $\mechc$ within the family of all  distributions $\dists$  is at most $\frac{\mu}{\lambda}$, i.e., $\poa(\mechc, \dists) \leq \frac{\mu}{\lambda}$.
%\end{theorem}
\ignore{% this is old:
\subsection{Corollaries of the Main Results}
\yl{remove entire section?}
Next we present some examples illustrating the power of the results of \Cref{thm:smooth imply poa combined} and \Cref{thm:semi-smooth imply poa combined} in proving PoA bounds for many auctions, in the presence of a  secondary market that is a trade mechanism.

We start with first-price auctions and all-pay auctions for the single-item setting.
\begin{theorem}[\citealp{roughgarden2012price}]\label{thm:single item}
For single-item setting {with independent prior distributions},
the first-price auction is $(1-\sfrac{1}{e}, 1)$-smooth
and all-pay auction is $(\sfrac{1}{2}, 1)$-smooth.
\end{theorem}
From these smoothness bounds, by Theorem \ref{thm:smooth imply poa combined} we immediately get the following corollary for first-price auction and for all-pay auctions, with independent prior distributions:
\begin{corollary}\label{cor:FPA-ind}
Consider the single-item setting with independent prior distributions.
% Fix any signaling protocol $\Gamma$ and any trade mechanism $\mechs$.
%% Fix any secondary market $\mechs$ satisfying voluntary participation and weak budget balance.
If $\mechf$ is the first-price auction then
for  any signaling protocol $\Gamma$ and any trade mechanism $\mechs$,
the combined market $\combinedGame$
%the mechanism that combines the first-price auction with $\mechs$
is $(1-\sfrac{1}{e}, 1)$-smooth and it has price of anarchy at most $\sfrac{e}{(e-1)}$.
Similarly, if $\mechf$ is the all-pay auction then the combined market $\combinedGame$
 is $(\sfrac{1}{2}, 1)$-smooth and it has price of anarchy at most $2$.
% The price of anarchy of the market combining the first-price auction with $\mechs$ is at most $\sfrac{e}{(e-1)}$,
%and the price of anarchy of the market combining all-pay auction  with $\mechs$ is at most $2$.
\end{corollary}

As shown in \citet{syrgkanis2013composable},
the above theorem can be directly generalized to the combinatorial auction settings
by running first-price auction or all-pay auction simultaneously on each item
when agents have monotone submodular valuations.
This extension is straightforward,
and hence the details are omitted in this paper. \mbc{it should be added explicitly. Also, this seems to be a stronger result than the one for multi-unit (\cref{cor:discriminatory auction}) as it holds even if items are different, but with the same smooth parameters. am I missing anything? } \bjl{If I understand correctly, the two results are for different auction formats. I.e., simultaneous item price auctions applied to homogeneous items isn't the same as the discriminatory auction.}



% First we consider the multi-item setting,
% where the feasibility constraint $\feasibles$ in this setting is that
% each item is allocated to at most one agent.
% We assume agents have submodular valuations,
% i.e.,
% for any agent $i$, any type $\type_i$,
% any sets $X_1, X_2 \subseteq [m]$, we have
% $\val_i(X_1;\type_i) + \val_i(X_2;\type_i) \geq
% \val_i(X_1\cap X_2;\type_i) + \val_i(X_1\cup X_2;\type_i)$.
% Here $m$ is the number of items holden by the seller.
% Moreover, we assume agents have monotone valuations,
% i.e.,
% for any agent $i$, any type~$\type_i$,
% any sets $X_1\subseteq X_2 \subseteq [m]$, we have
% $\val_i(X_1;\type_i) \leq \val_i(X_2;\type_i)$.
% In this setting, we consider two different auction mechanisms:
% (1) the simultaneous first-price auction,
% where each agent simultaneously announces her bids for each item,
% the mechanism allocates each item to the highest bidder,
% and charges the agents their bids for each winning item;
% (2) the simultaneous all-pay auction, where each agent simultaneously announces her bids for each item,
% the mechanism allocates each item to the highest bidder,
% and charges the agents their bids for all items.

% \begin{theorem}[\citealp{syrgkanis2013composable}]\label{thm:submodular}
% For multi-item setting with monotone submodular valuations,
% simultaneous first-price auction is $(1-\sfrac{1}{e}, 1)$-smooth
% and simultaneous all-pay auction is $(1-\sfrac{1}{2}, 1)$-smooth.
% \end{theorem}

% \begin{corollary}
% For multi-item setting with monotone submodular valuations,
% given any secondary market satisfying voluntary participation and weak budget balance,
% the price of anarchy is at most $\sfrac{e}{(e-1)}$ for simultaneous first-price auction
% and at most $2$ for simultaneous all-pay auction
% when the prior distributions are independent.
% \end{corollary}

% Another example is the multi-unit setting.
% Here we have $m$ units of the same item
% and the feasibility constraint is that
% the total units sold to all agents is at most $m$.
% In this setting, the valuation of the agent for any allocation is uniquely determined by the number of units she receives in the allocation.
% In addition to monotone submodular valuations,
% here we also consider monotone subadditive valuations,
% i.e.,
% for any agent $i$, any type $\type_i$,
% any sets $X_1, X_2 \subseteq [m]$, we have
% $\val_i(X_1;\type_i) + \val_i(X_2;\type_i) \geq
% \val_i(X_1\cup X_2;\type_i)$.
% The mechanism we adopt here is the discriminatory auction,
% a generalization of first-price auction.
% Here each agent report her marginal value for each additional unit,
% the mechanism find the welfare maximization allocation,
% and charges the agents their bids for each additional unit they receive.

Another example is the multi-unit setting with decreasing-marginal valuations.
The mechanism we adopt here is the discriminatory auction,
a generalization of first-price auction.
Here each agent report her marginal value for each additional unit,
the mechanism finds the reported-welfare-maximizing allocation,
and charges the agents their bids for each additional unit they receive.


\begin{theorem}[\citealp{de2013inefficiency}]\label{thm:submodular multi-unit}
For the multi-unit setting {with independent prior distributions},
over decreasing-marginal valuations, the discriminatory auction is $(1-\sfrac{1}{e}, 1)$-smooth.\footnote{
The authors also showed that if the valuations are monotone subadditive, then the mechanism is $(\frac{1}{2}(1-\sfrac{1}{e}), 1)$-smooth.\mbc{why not have this as a theorem ?}}
\end{theorem}

% \begin{theorem}[\citealp{feldman2013simultaneous}]\label{thm:subadditive}

% \end{theorem}
%By Theorem \ref{thm:smooth imply poa combined} we get:
From this smoothness bound, by Theorem \ref{thm:smooth imply poa combined} we immediately get:
\begin{corollary}\label{cor:discriminatory auction}
Consider the multi-unit setting with independent prior distributions over decreasing marginal valuations.
%Fix any signaling protocol $\Gamma$ and any trade mechanism $\mechs$.
%Fix any secondary market $\mechs$ satisfying voluntary participation and weak budget balance.
If $\mechf$ is the discriminatory auction then for  any signaling protocol $\Gamma$ and any trade mechanism $\mechs$,
the combined market $\combinedGame$ is $(1-\sfrac{1}{e}, 1)$-smooth and it has price of anarchy  at most $\sfrac{e}{(e-1)}$.
% The price of anarchy of the market combining the discriminatory auction with $\mechs$ is at most $\sfrac{e}{(e-1)}$.
\end{corollary}

\mbc{add more corollaries, for Combinatorial Auctions, generalized second price etc.}

We next move to using \Cref{thm:semi-smooth imply poa combined} to prove PoA bounds for correlated prior distributions.
We show that the combined market running first-price auction with a secondary market
has small price of anarchy.%  for any correlated distribution given any secondary market satisfying voluntary participation and weak budget balance.

\begin{theorem}[\citealp{roughgarden2017price}]
For the single-item setting with any prior distribution, the first-price auction is $(1-\sfrac{1}{e}, 1)$-semi-smooth.
\end{theorem}

From this semi-smoothness bound, by \Cref{thm:semi-smooth imply poa combined} we immediately get:
\begin{corollary}\label{cor:FPA-cor}
Consider the single-item setting with any prior joint distribution (possible correlated).
If $\mechf$ is the first-price auction then for  any signaling protocol $\Gamma$ and any trade mechanism $\mechs$,
the combined market $\combinedGame$ is
%Fix any trade mechanism $\mechs$.
%%Fix any secondary market $\mechs$ satisfying voluntary participation and weak budget balance.
%Then for any signaling protocol $\Gamma$,
%% The price of anarchy of the market combining the first-price auction with $\mechs$ is at most $\sfrac{e}{(e-1)}$.  Then
%the mechanism  that combines the first-price auction with $\mechs$ is
$(1-\sfrac{1}{e}, 1)$-semi-smooth, and it has price of anarchy at most $\sfrac{e}{(e-1)}$.
\end{corollary}
%\mbc{This seems to dominate the result \Cref{cor:FPA-ind}. Are the smooth parameters indeed the same?}
%\yl{For first price this is indeed stronger than \Cref{cor:FPA-ind}. But we can get all pay for smoothness as well, while not for semi-smooth. } \mbc{I see. seems like we should keep the FPA part of \Cref{cor:FPA-ind} as we talk about its extension to submodular (will such extension work even for correlation using this corollary about FPA instead of \Cref{cor:FPA-ind}? If so, we should state it.) In the meanwhile, I have added a sentence below }\yl{I think semi-smooth does not extend to simultaneous mechanism in submodular setting. That's my understanding.}
%%For the single-item setting, given any secondary market satisfying voluntary participation and weak budget balance, the price of anarchy is at most $\sfrac{e}{(e-1)}$ for first-price auction when the prior distributions are correlated.

Note that this result for first-price auctions is stronger than the one presented in \Cref{cor:FPA-ind}, as it holds for any prior value distribution, not only when valuations are independent across the agents.
} % ignore


==> content/symmetric.tex <==
% \section{Secondary Markets for the Single Item Setting}
% In this section we present some additional result for the single item setting.
% We first present efficiency result for two agents with i.i.d.\ value distributions,
% proving that all equilibria in the combined markets are efficient for first-price and all pay auctions.
% We then show that
% when the bids in the auction are not revealed in the secondary market,
% for first-price or second price auction
% with anonymous reserve,
% the price of anarchy for revenue is at least~$2.62$.

\section{Efficiency in Single-Item Symmetric Environments}
\label{sec:symmetric}
%We have seen in \cref{sec:smooth} %\Cref{example:FPA-welfare-loss} 
%that equilibrium  welfare of a combined market can sometimes be lower than the (unique) equilibrium welfare of the stand-alone auction, without the aftermarket. % (Example \ref{example:FPA-welfare-loss}).
%We have seen that a combined market, an auction combined with a trade mechanism as a secondary market, can sometimes have lower welfare than the welfare of the stand-alone auction (Example \ref{example:FPA-welfare-loss}).
%While 
We have shown that the welfare loss is bounded for smooth auctions (\Cref{sec:smooth}).
In this section, we are interested in understanding conditions under which there will not be any welfare loss.
We present such conditions for some single-item auctions (e.g., first-price auctions),\footnote{Second-price auctions have multiple Nash equilibria, so equilibrium selection is an issue there, even within a standalone market.} 
in the well-studied case of two agents with i.i.d.\ valuation distributions.
Note that without information acquisition and aftermarkets, 
\citet{chawla2013auctions} show that for symmetric distributions, 
the first-price auction has a unique equilibrium, and it is efficient.

%We will focus on first-price auction in the single-item setting.
% \mbc{seems to me that this entire paragraph should be erased as a better motivation is presented in the second paragraph:}
% In \citet{garratt2006speculation},
% the authors showed that the efficiency guarantee of the first-price auction is not robust
% in the presence of secondary market
% if there is a speculator.
% In their model, they assume that the speculator has public valuation $0$ for the item.
% In this section, we will show that speculation does not deteriorate the efficiency guarantee for first-price auction
% if the valuation distribution of all buyers (including the speculator) are symmetric,
% and this result is robust to any form of the secondary market, including asymmetric secondary markets.
% % \mbc{Maybe we should remark that for IID bidders there is a unique NE in FPA that is monotone and thus efficient, so the PoS of any combined market running FPA and then an some mechanism $M_2$ that is weakly BB and IR is 1. This is so as the original NE is still NE with no trade in the secondary market. \\ Was the IID setting studied? Are there asymmetric equilibria? }

%\subsection{Pre-market}
%With the investment incentives, even if agents have no private information in ex ante (hence there is no need for information acquisition)
%and there is no aftermarket, 
%for first-price auction, 
%the equilibrium outcome \mbc{is it unique?} may not be efficient.
%
%\begin{example}
%Consider a the single-item setting with two i.i.d.\ buyers. 
%Each buyer can choose not to invest (pay cost $0$) with value $0$, 
%or invest (pay cost $1$) with value $2$. 
%In the optimal welfare is $1$, where exactly one buyer invests and the buyer who invests wins the item. 
%
%Here is a symmetric equilibrium of the buyers. 
%Each buyer invest with probability $\frac{1}{2}$. 
%When the buyer does not invest, the bid is $-1$ and the buyer will not win the item with probability $1$.
%When the buyer invests, the buyer bids according to distribution $F$ with cumulative probability $F(b) = \frac{2}{2-b}-1$. 
%It is easy to verify that this is an equilibrium strategy for both buyers 
%and the equilibrium welfare is $\frac{3}{4}$.
%\end{example}

\subsection{Information Acquisition}
\label{sec:symmetric info acq}
When the auction is the first-price auction and the agents can acquire costly information about opponents, even in symmetric environments when there is no aftermarket, 
there may exist equilibria that are not efficient. 
%\mbc{it will be nice to have a strong result - a setting in which {\bf every} symmetric equilibrium is not efficient. Is this the case for this example? Maybe we can show that if the other agent does not acquire information, the agent is better off deviating. If the result does not hold for this example, can we find a different one with that property?}
This is formally shown in \cref{exp:info acquire symmetric}.
Intuitively, this holds because although additional information is not beneficial in the social planner's perspective, 
it is profitable for each individual to acquire information for better bidding strategies.
In the following proposition we state a stronger result, showing that any equilibrium in \cref{exp:info acquire symmetric} is inefficient. 
The proof is deferred in \cref{apx:proof efficient}.

\begin{restatable}{proposition}{leminefficient}\label{lem:symmetric inefficiency}
There exists a single-item setting with two i.i.d.\ buyers such that 
with information acquisition, 
the allocation of any equilibrium is inefficient.
% or: \mbe{the welfare of any equilibrium is not maximized (any equilibrium is  inefficient)}. %MB: welfare cannot be efficient. 
%OLD: the welfare in any equilibrium is efficient
\end{restatable}

%\begin{example}
%Consider selling a single item to two i.i.d.\ buyers
%using first-price auction. 
%With probability $\frac{1}{2}$, the value of the buyer is $0$, 
%and with rest probabilities, the value of the buyer is drawn from uniform distribution supported on $[0,1]$. 
%For each buyer $i\in\{1,2\}$ with value $\val_i\in[0,1]$, 
%she can choose to not acquire any information,
%or pay cost $\frac{v^2_i}{16}$ to observe whether the opponent has value $0$ or not.
%
%Here is a symmetric equilibrium of the buyers. 
%For each buyer $i\in\{1,2\}$ with value $\val_i\in[0,1]$, 
%if $\val_i=0$, the buyer will not acquire any information 
%and opt out of the auction (e.g., bid $-1$ which is below the minimum acceptable bid of $0$).
%%bid $-1$ in the auction \mbc{if the other agent bids $-1$, then it seems better to bid $-0.99$ when the value is 0. I am confused by the claim this is  an equilibrium}.\yl{I implicitly set a reserve price 0 for the first price auction. Also here we can let agent with bid 0 to bid 0 and carefully design the tie-breaking rule, but I prefer not doing that.}
%% MB: trying to make this explicit. 
%If $\val_i>0$, the buyer will acquire information with cost $\frac{v^2_i}{16}$, 
%bid $0$ if opponent has value $0$, 
%and bid $\frac{\val_i}{2}$ otherwise.
%It is easy to verify that this is an equilibrium strategy for both buyers 
%and the equilibrium welfare is sub-optimal as agents pay positive costs for acquiring additional information.
%\end{example}


\subsection{Aftermarkets}
%We consider the setting of a seller that has a single item for sale, and two buyers with i.i.d.\ valuation distributions.

%\mbc{revised this paragraph:}
%\mbe{While we saw that 11111111111}
In \citet{hafalir2008asymmetric},
the authors consider the setting with two i.i.d.\ agents
and show that when combining the first-price auction with a secondary market taken from a specific family of secondary markets\footnote{Essentially, in the model of \citet{hafalir2008asymmetric},
the agent winning the item in the auction posts a price to the other agent in the secondary market.
}, assuming bids in the auction are not revealed before the secondary market, any BNE of the combined market in which bids in the auction are non-decreasing is welfare-maximizing.
%the equilibrium in the combined market is efficient if (1) actions are not revealed in the secondary market, and (2) the bids in the auction are non-decreasing.
We generalize their BNE efficiency result by showing it holds under significantly weaker conditions.  First, our result allows the aftermarket to be any trade mechanism that satisfies ex post individual rationality %with the additional mild assumption of ex post individual rationality of the aftermarket mechanism
(\Cref{def:ex post participate}).
%\footnote{
%Note that this assumption is sufficient to capture natural secondary markets such as winner in the auction posting price to other players in the secondary markets,
%or where the agents agree on the Nash bargaining solution.
%Essentially we want to exclude situations where items are sometimes traded from high-value agents to low-value agents in the secondary markets.
%For example, consider the case with two players where
%player 1 with value 2 wins the item and thinks player 2 has value 1 or 3 with probability $\frac{1}{2}$ each.
%In the secondary market, both agents can only choose to opt in or not.
%If both opt in, the item goes to player 2, and player 2 pays her value to agent~1.
%Note that this does not satisfy ex post individual rational but does satisfy voluntary participation.
%The fact it sometimes results with inefficient allocation shows voluntary participation is not sufficient for the claim  to hold.
%}
% MB: removed as "trade mechanism" already includes is:
% and weak budget balance.
Second, we allow arbitrary information about bids, outcomes, and payments of the auction to be revealed before the secondary market.
%make weaker assumptions on the information revealed before the secondary market, allowing information, as the bids in the auction, to be partially or fully revealed.
Given this information agents update their belief about others' valuation.
As in \citet{hafalir2008asymmetric}, we consider only strategies in which
%(1) valuations of the agents are not directly revealed before the secondary market and cannot be deduced beyond what is implied by the bids (\Cref{asp:no value reveal});
the bids in the auction are non-decreasing.\footnote{We conjecture that this assumption is unnecessary and that any BNE of the combined market is efficient, even without this assumption.}
% Our result applies to all secondary markets satisfying ex post individual rational and weak budget balance.
% and a weak ex post condition specified in \Cref{asp:ex post trade}.
The techniques we use in the proof are similar to the techniques in \citet{chawla2013auctions}.
It shows that any monotone strategies must be essentially identical.

% OLD:
% The techniques used in this section is similar to \citet{chawla2013auctions},  where the authors showed that the unique equilibrium for first-price auction is efficient for symmetric distribution if there is no secondary market.



% \begin{assumption}\label{asp:ex post trade}
% For any valuation profile of the agents,
% no trade occurs in the secondary market if the allocation in the auction is efficient.
% \end{assumption}
% Note that under voluntary participation and weak budget balance,
% if the allocation is efficient in ex ante,
% then no trade occurs for all valuation profiles.
% \Cref{asp:ex post trade} is stronger than that,
% which exclude situations where the allocation is efficient only for some valuation profiles,
% while trade can still occur for those efficient allocations since all agents only maximize their utilities in expectation.
% However, this assumption is sufficient to capture natural secondary markets such as winner in the auction posting price to other players in the secondary markets,
% or where the agents agree on the Nash bargaining solution.

% \mbc{this is rather weak version of ex post individual rational- 1) it only need to hold in equilibrium, and not for any profile of actions of the others. 2) it is in expectation over the strategies of the agents, not for any realized actions 3) it is in expectation over randomness of the mechanism and not every realization of it. Is this indeed the intention? Maybe we should remark about this. } \mbc{what about ex-post BB? Aren't we using it at the end?}\yl{To address the three questions: (1) the voluntary participation is a property on the pair of action and type, and certainly we cannot define it for all possible pairs. Thus define it for the equilibrium strategy is proper here.  (2,3) Yes expectation over strategy and mechanism is sufficient here. Essentially ex post just mean ex post over valuation profile. Finally, we do not have ex-post BB since we already define BB in an ex post matter in definition 3.}


%\mbc{An issue we need to discuss: in the theorem below, as well as other results, we never claim that an equilibrium actually exists.  }
%\yl{There is at least one equilibrium where agents adopt symmetric strategies in the first market, allocation is efficient,
%and no trade occurs in secondary market.}\mbc{added this as a footnote here. We need to discuss if we can say anything general that hold for the other results.}
\begin{restatable}{theorem}{thmefficient}\label{thm:symmetric efficiency}
Consider the  single-item setting with two i.i.d.\ buyers with atomless and bounded valuation distribution that has positive density everywhere on the support.
Fix the auction $\mechf$ to be either the first-price auction or the all-pay auction. Fix any signaling protocol $\Gamma$ and
any trade mechanism satisfying  ex post individual rationality.
Then  in the combined market $\combinedGame$,
every Bayesian Nash equilibrium\footnote{Note that there is at least one efficient equilibrium:  agents adopt symmetric strategies in the auction, the resulting auction allocation is efficient,
		and no trade occurs in the secondary market.} in which the bids of the agents in the auction are non-decreasing in values, is efficient.
% OLD:
%if bids in the auction environment are non-decreasing in values then all Bayesian Nash equilibria\footnote{Note that there is at least one efficient equilibrium:  agents adopt symmetric strategies in the auction, the resulting auction allocation is efficient, 	and no trade occurs in the secondary market.} are efficient, i.e., the price of anarchy is $1$.
\end{restatable}
\begin{figure}[t]
\centering
\input{fig/symmetric}
\vspace{-6pt}
\caption{\label{f:symmetric dist}
Asymmetric bid functions $\bid_1$ and $\bid_2$.
}
\end{figure}

%\yl{added sketch for the proof.}\mbc{made minor edits.}
We next briefly outline the proof of \cref{thm:symmetric efficiency}; the full proof appears in  \cref{apx:proof efficient}.
Observe first that if the agents use symmetric strategy profiles in the auction
then the allocation of the auction is efficient,
and thus by voluntary participation of the secondary market
the outcome of the combined market will be efficient as well.
So let's assume the bids are not symmetric.

For the given strategies of the agents in the combined market, we denote by $\util_i(v)$ the expected utility of agent $i\in \{1,2\}$ after the aftermarket , given that the agent's value is $v$.
Suppose there exists a value $\val^*$ such that the bid of agent $1$ with value $\val^*$ in the auction is higher than that for agent $2$ with the same value.
Consider the maximum-length interval $(\bar{\val}, \bar{\val}')$
such that the bid of agent $1$ is always weakly higher than agent $2$ for values within the interval.
Since the secondary market satisfies ex post individual rationality,
the interim allocation in the combined market for agent $1$ between $(\bar{\val}, \bar{\val}')$
is higher than agent $2$,
which implies that the expected
%\mbc{are we talking about the utilities in combined market? need to say this explicitly. added a sentence above.}
utility difference satisfies
$u_1(\bar{\val}') - u_1(\bar{\val})
\geq u_2(\bar{\val}') - u_2(\bar{\val})$
by the characterization in \cite{myerson1981optimal}.
Moreover, through the payment format of first-price auction or all-pay auction,
since the secondary market is a trade mechanism,
we can additionally conclude that
$u_1(\bar{\val}) \geq u_2(\bar{\val})$ and
$u_1(\bar{\val}')\leq u_2(\bar{\val}')$.
Thus we can conclude that $u_1(\bar{\val}') - u_1(\bar{\val})
= u_2(\bar{\val}') - u_2(\bar{\val})$,
and the only possible situation for the equality to hold is that the item is resold in the secondary market such that
the allocation is efficient.

%MB: removed, leaving only the footnote:
%Note that in the statement of the theorem, we make the assumption of non-decreasing bids. We conjecture \mbc{this conjecture also appears as footnote 14, so one of the two appearances should be removed (probably the footnote).}\bjl{I actually prefer removing this paragraph and keeping the footnote.  I added a bit more text to the footnote.} that this assumption is not necessary, and that any BNE of the combined market is efficient, even without this assumption.

%\begin{proof}[Proof of \Cref{thm:symmetric efficiency}]
%%	\mbc{add an explicit reference in the proof to the point in which the "valuation distribution that is continuous on a bounded interval" assumption is used. }
%%	\yl{This assumption is not necessary. I think I added it for convenience in previous proof, and can be removed here.}\mbc{ok, I have removed the assumption from the new version of the theorem. please verify the proof indeed never uses it.}
%	
%Since the secondary market satisfies
%ex post individual rational and weak budget balance,
%for any valuation profile such that the allocation in the auction environment is efficient,
%no trade occurs in the secondary market,
%and hence the allocation is efficient in the combined market.
%If both agents use the same strictly increasing strategy,
%the allocation is efficient in the auction environment for all valuation profiles,
%and hence it is efficient in the combined market.
%Moreover, if both agents use the same monotone strategy while there exists an interval $(\val',\val'')$ with the same bid $b''$ for all values in this interval,
%%for each value $\val \in (\val',\val'')$,
%%the utility of agent with value $\val$ is at least $(\val - b'' -\epsilon) \cdot F(\val'')$
%%for any $\epsilon >0$ by bidding $b''+\epsilon$ in the auction and opt out the secondary market.
%%Note that the
%at least one agent with value in the interval can strictly increase her bid by an infinitesimal amount to strictly increase her utility,
%contradicting to the assumption that the strategies are sustained under equilibrium.
%
%We next assume that strategies of the two agents are monotone yet asymmetric.
%For any value $\val^*$ such that $\bid_1(\val^*) > \bid_2(\val^*)$,
%let $\bar{\val}\leq \val^*$ be the infimum value such that $\bid_1(\bar{\val}) \geq \bid_2(\bar{\val})$,
%and $\bar{\val}'\geq \val^*$ be the supremum value such that $\bid_1(\bar{\val}') \geq \bid_2(\bar{\val}')$.
%This is illustrated in \Cref{f:symmetric dist}.
%{The definition of $\bar{\val}$ implies that there exists $\epsilon' > 0$
%such that $\bid_2(\val) > \bid_1(\val)$ for
%any $\val\in(\bar{\val}-\epsilon', \bar{\val})$.
%This further implies that
%$\lim_{\val\uparrow\bar{\val}} \bid_2(\val)
%\geq \lim_{\val\uparrow\bar{\val}}\bid_1(\val)$.}
%% First we show that $\util_1(\bar{\val}) = \util_2(\bar{\val})$
%% and $\util_1(\bar{\val}') = \util_2(\bar{\val}')$.
%
%First we show that {$\util_1(\bar{\val}) \geq \util_2(\bar{\val})$.
%The claim that $\util_1(\bar{\val}') \leq \util_2(\bar{\val}')$ holds similarly. }
%We claim that
%$\lim_{\val\uparrow\bar{\val}} \bid_1(\val)
%= \lim_{\val\uparrow\bar{\val}}\bid_2(\val)$.\footnote{$\lim_{\val\uparrow\bar{\val}}$ means taking the limit as $\val$ increases to $\bar{\val}$ (limit from below).}
%Recall that $\lim_{\val\uparrow\bar{\val}} \bid_2(\val)
%\geq \lim_{\val\uparrow\bar{\val}}\bid_1(\val)$ and assume in contradiction that
%$\epsilon = \lim_{\val\uparrow\bar{\val}} \bid_2(\val)
%- \lim_{\val\uparrow\bar{\val}}\bid_1(\val)>0$.
%%OLD:
%%Suppose in contradiction that $\lim_{\val\uparrow\bar{\val}} \bid_2(\val) > \lim_{\val\uparrow\bar{\val}}\bid_1(\val)$
%%%\mbc{this seems to be with loss of generality. Don't we need to also take care of the case $\lim_{\val\uparrow\bar{\val}} \bid_1(\val) < \lim_{\val\uparrow\bar{\val}}\bid_2(\val)$? }
%%%\yl{Argument for $\lim_{\val\uparrow\bar{\val}} \bid_1(\val) < \lim_{\val\uparrow\bar{\val}}\bid_2(\val)$ is identical.}\mbc{note that the bidders are not symmetric as we define $\bar{\val}$ to satisfy $\bid_1(\bar{\val}) \geq \bid_2(\bar{\val})$. Please add a short description about the proof of this case (we switch the roles of the agents, right?).}
%%%\yl{But the proof does not require this information. For this other case, just following exactly the same argument, we can show that if $\lim_{\val\uparrow\bar{\val}} \bid_1(\val) < \lim_{\val\uparrow\bar{\val}}\bid_2(\val)$,
%%%there exists a deviating strategy for player 2 (decrease the bid by $\frac{\epsilon}{2}$) that generates higher utility.}
%%and let  $\epsilon = \lim_{\val\uparrow\bar{\val}} \bid_2(\val)  - \lim_{\val\uparrow\bar{\val}}\bid_1(\val)$. Note that by assumption $\epsilon>0$.
%There exists a value $\hat{\val}_2$ for agent $2$ satisfying
%$\hat{\val}_2 \in (\bar{\val}-\frac{\epsilon}{4}, \bar{\val})$
%such that
%$\bid_2(\hat{\val}_2) \in
%[\lim_{\val\uparrow\bar{\val}}\bid_2(\val) - \frac{\epsilon}{2},
%\bid_2(\bar{\val})]$.
%%\yl{and $\Pr_{v\sim F_2}[\hat{\val} \leq v \leq \bar{v}] \leq \frac{\epsilon \cdot F_2(\bar{v})}{4\bar{v}}$}.
%%\mbc{$\val$ is in use, so we should replace the variable in the limit: $\lim_{\val\uparrow\bar{\val}}\bid_1(\val) $ better be $\lim_{\tilde{\val}\uparrow\bar{\val}}\bid_1(\tilde{\val})  $ }.
%Thus agent 2 with value $\hat{\val}_2$ can lower her bid $\bid_2(\hat{\val}_2)$ by $\frac{\epsilon}{2}$ without affecting the allocation in the auction,
%and increase the utility in the auction environment by $\frac{\epsilon}{2}$ when she wins the item.
%Thus in any case she wins with bid $\bid_2(\hat{\val}_2)$,
%her utility from deviating and bidding $\bid_2(\hat{\val}_2)-\frac{\epsilon}{2}$ instead, is at least $\hat{\val}_2 - \bid_2(\hat{\val}_2) + \frac{\epsilon}{2}$ in the auction, and this cannot decrease in the combined market as the secondary market satisfies \yl{voluntary participation.}
%%ex post individual rational.
%
%We next argue that her utility in the combined market when bidding $\bid_2(\hat{\val}_2)$ in the auction is at most $\hat{\val}_2 - \bid_2(\hat{\val}_2) + \frac{\epsilon}{4}$, and thus smaller than with the deviation.
%Indeed, if she wins with bid $\bid_2(\hat{\val}_2)$ in the auction, her utility from the auction is $\hat{\val}_2 - \bid_2(\hat{\val}_2)$,
%and if she end up reselling the item in the secondary market,
%as it satisfies ex post individual rational and weak budget balance,
%her additional utility is bounded by
%$ {\val}_1-\hat{\val}_2 $, where $\val_1$ is the value of agent $1$.
%To complete the proof we show that when agent $2$ wins in the auction with bid $\bid_2(\hat{\val}_2)$ it holds that ${\val}_1\leq \bar{\val}$, and this will prove the claim since $\val_1-\hat{\val}_2\leq \bar{\val}-\hat{\val}_2\leq \frac{\epsilon}{4}$.
%
%Note that if $\bid_1(\val) > \bid_2(\hat{\val}_2)$ for any $\val > \bar{\val}$, the above claim holds.
%Otherwise, let $\epsilon''>0$ be the supremum value such that $\bid_1(\val) \leq \bid_2(\hat{\val})$ for any $\val \in [\bar{\val}, \bar{\val} + \epsilon'')$. % the supremum on gives the open interval from above.
%Moreover, by the assumptions we made on the equilibrium strategy, we have
%$\bid_1(\val) \geq \bid_2(\val) \geq \bid_2(\hat{\val})$
%for any $\val \in [\bar{\val}, \bar{\val} + \epsilon'')$.
%Thus $\bid_1(\val) = \bid_2(\val)= \bid_2(\hat{\val})$
%for any $\val \in [\bar{\val}, \bar{\val} + \epsilon'')$.
%First we claim that $\bid_2(\hat{\val}) < \bar{\val} + \epsilon''$.
%This is because otherwise for agent $2$ with value $\hat{\val}$,
%her utility under equilibrium is negative since conditional on winning,
%her payment in the auction is at least $\bar{\val} + \epsilon''$,
%the value of agent $1$ is $\val_1 \leq \bar{\val} + \epsilon''$ (as agent 1 losses the auction),
%and strictly smaller with positive probability, % \mbc{why?}\yl{with additional continuity assumption added to statement, this holds since $v< \bar{\val} + \epsilon''$ has positive measure.},
%and the payment from resale is at most $\val_1$.
%In the case that $\bid_2(\hat{\val}) < \bar{\val} + \epsilon''$,
%there exists sufficiently small $\delta>0$
%such that agent $2$ with value $\bar{\val} + \epsilon''-\delta$
%%\mbc{I think there might be some subtle issue here. The tie in bids is only for $\val \in [\bar{\val}, \bar{\val} + \epsilon'')$, so the interval is open at the top and there might not be a tie there. Seems like we can only argue this claim for value slightly below the top.}\yl{I think arguing this for value $\bar{\val} + \epsilon''-\delta$ with arbitrarily small $\delta$ will resolve your concern?} \mbc{yes, I think so.}
%can simply increase the bid by an infinitesimal amount, which would win the item for all opponent's value $\val_1< \bar{\val} + \epsilon''$, which increases her utility.
%Therefore, we must have $\lim_{\val\uparrow\bar{\val}} \bid_1(\val) = \lim_{\val\uparrow\bar{\val}}\bid_2(\val)$,
%and we define the limit as~$\bid^*$.
% %\mbc{do we know this even has positive probability? }\yl{This happens with positive probability since we are considering continuous distribution with positive density everywhere.}
%
%
%%As illustrated in the first paragraph,
%%there exists an agent \mbc{I think this must holds for agent with the highest value $\bar{\val} + \epsilon''$ } with value between $[\bar{\val}, \bar{\val} + \epsilon'']$
%%that can benefit from increasing the bid by an infinitesimal amount \mbc{seems like this can only be true if the bids are strictly below the value. Do we know they are not equal? }
%%\yl{Yes this is because if this bid is higher than $\bar{\val} + \epsilon''$,
%%then the utility of agent with value $\bar{\val}$ would be negative.}\mbc{this seems true in the auction, but maybe resale can increase the utility enough? explain this point in the proof.}, \yl{Since higher value agents will bid higher, under equilibrium, conditional on agent with value $\val < \bar{\val} + \epsilon''$ winning, the value of the opponent is at most $\bar{\val} + \epsilon''$. \mbc{I think that for this to hold we need to define $\epsilon''$ to be the supremum  such that the bid at value $\bar{\val} + \epsilon''$ is the same as the bid in $\bar{\val}$. I do not see how this works without this }
%%Thus the resale in secondary market will not be able to cover the loss in the auction. }
%%contradicting to the assumption that $\bid_1,\bid_2$ can be sustained under equilibrium.
%%}
%
%%\mbc{please add a proof that "when agent $1$ wins in the auction with bid $\bid_1(\hat{\val})$ it holds that ${\val}_2\leq \bar{\val}$". The proof should be robust to switching the role of the agents, although bidders are not symmetric as we define $\bar{\val}$ to satisfy $\bid_1(\bar{\val}) \geq \bid_2(\bar{\val})$}
%%\yl{This is because by the assumptions we made on the equilibrium and the definition of $\bar{v}$,
%%we know that $\bar{v}$ is the supreme value of agent 2 that can bid above $\lim_{\val\uparrow\bar{\val}} \bid_1(\val)\geq\bar{\val}$.}\mbc{but this seems like an argument that does depend on the asymmetry of the condition $\bid_1(\bar{\val}) \geq \bid_2(\bar{\val})$. Pleasw write a full argument that does not depend on this.}
%%Indeed if agent $1$ wins in the auction with bid $\bid_1(\hat{\val})$ and  ${\val}_2> \bar{\val}$, then FINISH!
%
%%Indeed, if ${\val}_2> \bar{\val}$ then by definition of $\bar{\val}$, in such case agent $2$ bids at least $b_2(\bar{\val})$ and must win as agent $1$ bids only  $\bid_1(\hat{\val}_1) < \bid_1(\bar{\val}) \leq  \bid_2(\bar{\val})$.
%
%
%%\mbc{I have revised the proof, see above. This is the OLD stuff :}
%%%, in contradiction to the bid $\bid_1(\hat{\val})$ being a best response.
%%%\mbc{I do not think this is enough to get a contradiction, as the probability that the value is exactly $\val$ is zero. We need to argue that due to monotonicity there is a positive interval for which there is a positive gain by lowering the bid.}\yl{It doesn't matter if probability that the value is exactly $\val$ is zero. The equilibrium strategy should be optimal for all types including the ones appears with measure 0.}\mbc{I now realize the source of the problem. In the definition of a strategy being a best response, there are two options:  either taking expectation over types $\type_i$, or asking for it to hold for every realized $\type_i$. The definition we have takes expectation over $\dist$, so it matches the definition I had in mind, in which the best response is in expectation over types $\type_i$, not for every realized $\type_i$.  If so, bids of a zero measure  set of values have no influence on the expectation. We can consider changing the definition. What is the standard definition?} \yl{I think the interim version of the definition is more standard.}
%%We claim that this gain of at least $\frac{\epsilon}{2}$ is higher than her utility with the original bid $\bid_1(\hat{\val})$.
%%Indeed, since the secondary market satisfies ex post individual rational and weak budget balance,
%%when her value is~$\hat{\val}$ and she wins the item in the auction with bid $\bid_1(\hat{\val})$,
%%the utility for reselling the item in the secondary market is at most~$\frac{\epsilon}{4}$.
%%This holds as the bid of agent $2$ is at most $\bid_1(\hat{\val})$ when agent $1$ wins in the auction,
%%which implies that the value $\val_2$ of agent $2$ is at most $\bar{\val}$ since under equilibrium $b_2(v) \geq b_1(v) \geq b_1(\hat{v})$ for any $v\geq\bar{v}$.
%%By ex post individual rational and weak budget balance,
%%% the, and the payment of agent $1$ in the auction is at least ... , and thus
%%the payment of agent $1$ receives from resale is at most $v_2$,
%%%and since the difference in valuation between both players is $\val_2-\hat{\val}\leq \bar{\val}-\hat{\val}\leq \frac{\epsilon}{4}$,
%%and the utility increase of agent $1$ in the secondary market \mbc{I do not follow. We care about the total utility of agent 1 in the combined market. As agent 1 ends without the item, her utility is simply the difference in payments, which is at most $v_2-b_1(\hat{\val})$ (he will be paid at most $v_2$). But why do we claim that $v_2-b_1(\hat{\val})\leq \frac{\epsilon}{4}$? }
%%\yl{We are not claiming that $v_2-b_1(\hat{\val})\leq \frac{\epsilon}{4}$.
%%We NEVER directly bounding the utility in combined market.
%%The arguments is to prove the utility increase by entering secondary market is at most $\frac{\epsilon}{4}$.
%%To rephrase the whole paragraph,
%%the whole argument has following two steps. Let $u^*$ be the equilibrium utility in the first market and $p$ be the probability of winning in first market.
%%We have shown that by decreasing bid by $\frac{\epsilon}{2}$, the utility in first market increase by $\frac{\epsilon}{2}$ conditional on winning,
%%and hence the utility of deviation in combined market is at least $u^*+\frac{\epsilon p}{2}$
%%Then looking at the utility under equilibrium. Conditional on losing, the utility increase in secondary market is 0 since no trade occurs.
%%Conditional on winning, the utility increase in secondary market is at most $\frac{\epsilon}{4}$. Thus equilibrium utility is at most  $u^*+\frac{\epsilon p}{2}$, contradiction.
%%}
%%is
%%at most $\val_2-\hat{\val}\leq \bar{\val}-\hat{\val}\leq \frac{\epsilon}{4}$.
%%%Moreover, since $\Pr_{v\sim F_2}[\hat{\val} \leq v \leq \bar{v}] \leq \frac{\epsilon \cdot F_2(\bar{v})}{4\bar{v}}$,
%%%the probability of resale conditional on player $1$ winning the item is at most $\frac{\epsilon}{4\bar{v}}$,
%%%which implies that the expected utility gain from resale conditional on winning is at most
%%%$\frac{\epsilon}{4}$.
%%Hence it is strictly beneficial for her to deviate her bid,
%%a contradiction that $\bid_1, \bid_2$ are equilibrium strategies.
%
%
%
%\mbc{GOT TO HERE, PLEASE LEAVE THIS}
%
%For any $\delta > 0$,
%let $\delta' \in (0, \delta)$ be the constant such that $\bid_1(\val), \bid_2(\val) \in (b^*-\delta, b^*]$
%and $\bid_2(\val) > \bid_1(\val)$
%for any $\val \in (\bar{\val}-\delta',\bar{\val})$.
%The utility of agent 1 with any value $\val \in (\bar{\val}-\delta', \bar{\val})$ is
%\begin{align*}
%\util_1(\val) \geq (\val - b^* - \delta) \cdot \Pr_{\val\sim\dist_2}[\val \leq \bar{\val}]
%\geq (\bar{\val} - b_2(\val)) \cdot \Pr_{\val\sim\dist_1}[\val \leq \bar{\val}] - 3\delta
%\geq \util_2(\val) - 4\delta.
%\end{align*}
%The first inequality holds because player 1 can always choose to bid $b^*+\delta$
%and wins with probability at least $\Pr_{\val\sim\dist_2}[\val \leq \bar{\val}]$ in the auction,
%and retain at least the same utility in the combined market since the secondary market satisfies voluntary participation.
%The second inequality holds because $\bar{v} - \val \leq \delta'\leq \delta$, $b^*-b_2(v)\leq \delta$
%and $\Pr_{\val\sim\dist_1}[\val \leq \bar{\val}] = \Pr_{\val\sim\dist_2}[\val \leq \bar{\val}]$ due to the i.i.d.\ assumption.
%Moreover, similar to the argument in the previous paragraph,
%the payment to agent 2 from reselling the item to agent~1 is at most $\bar{\val}$,
%and the utility increase of agent 2 in the secondary market is at most $\delta'\leq\delta$.
%The latter implies the last inequality above.
%%The last inequality holds since agent 2 can only resell the item to agent 1 with payment below $\bar{\val}$ since
%%the secondary market satisfies ex post individual rational
%%and under equilibrium bid $\bid_2(\val)$,
%%she only wins the item if her opponent's value is below $\bar{\val}$.
%%Similarly, the utility of agent 2 with any value $\val \in (\bar{\val}-\delta', \bar{\val})$ is
%%\begin{align*}
%%\util_2(\val)
%%%\geq (\val - b^* - \delta) \cdot \Pr_{\val\sim\dist_1}[\val \leq \bar{\val}]
%%\geq (\bar{\val} - b_1(\val)) \cdot \Pr_{\val\sim\dist_2}[\val \leq \bar{\val}] - 3\delta
%%\geq \util_1(\val) - 4\delta.
%%\end{align*}
%%The first inequality holds by the same argument.
%%\yl{To be added.}
%%%Let $p_1$ be the probability that agent~$1$ wins in the auction,
%%%and $p_2$ be the probability that agent $1$ loses in the auction and the value of agent $2$ is at most $\bar{v}$.
%%%Note that $\bid_2(\val) > \bid_1(\val)$
%%%for any $\val \in (\bar{\val}-\delta',\bar{\val})$,
%%%when agent $1$ wins the item with value $\val$,
%%%the value of agent $2$ is smaller than $\val$.
%%%This implies that no trade occurs in the secondary market conditional on agent $1$ winning,
%%%and the event that the probability that agent $1$ wins in the auction
%%%is a subset of the event that value of agent $2$ is at most $\bar{v}$.
%%%Thus $p_1+p_2 = \Pr_{\val\sim\dist_2}[\val \leq \bar{\val}]$.
%%%Note that the utility of agent 1 conditional on winning the item is
%%%$\val-b_1(\val)$ since no trade occurs in the secondary market.
%%%The utility of agent 1 conditional on losing the item is at most
%%%$\val-\val_2$ since the secondary market satisfies voluntary participation.
%%%Thus the expected utility in the combined market is
%%%$p_1(\val-b_1(\val)) + p_2(\val-v_2)\leq (\val-b_1(\val))\Pr_{\val\sim\dist_2}[\val \leq \bar{\val}]$
%%%since $v_2\geq \bid_2(v_2)\geq \bid_1(\val)$.
%Hence $\lim_{\val\uparrow\bar{\val}} \util_1(\val) \geq \lim_{\val\uparrow\bar{\val}}\util_2(\val)$.
%Since the interim utility is a continuous function of the valuation, we have
%$\util_1(\bar{\val}) \geq \util_2(\bar{\val})$.
%
%% Both $\bar{\val}$ and $\bar{\val}'$ are finite and well defined since the support of the valuation distribution is bounded.
%
%
%%If the FPA is not efficient, then
%% Assume that there exists $\bar{\val} < \bar{\val}'$
%% such that $\bid_1(\bar{\val}) = \bid_2(\bar{\val})$,
%% $\bid_1(\bar{\val}') = \bid_2(\bar{\val}')$,
%% and $\bid_1(\val) > \bid_2(\val)$ for any $\val\in (\bar{\val},\bar{\val}')$.
%% % \mbc{will it always exist? what if not?}
%% We will show that in this case, the only possible scenario for the asymmetry in the bid functions is that
%% agents will re-trade in the secondary market such that the allocation is efficient.
%% Note that other cases such as bids $\bid_1(\val) > \bid_2(\val)$ for any $\val$ can be proved similarly.
%% Thus the proof for those special cases is omitted here
%% and the readers can refer to \citet{chawla2013auctions} for a detailed discussion.
%
%% First we show that $\util_1(\bar{\val}) = \util_2(\bar{\val})$
%% and $\util_1(\bar{\val}') = \util_2(\bar{\val}')$.
%% This is due to the format of the first-price auction.
%% Note that for each agent $i$, if $\val_i = \bar{\val}$,
%% then agent $i$ wins the item if and only if
%% her bid is higher than her opponent.
%% Since $\bid_1(\bar{\val}) = \bid_2(\bar{\val})$
%% and bids are monotone,
%% this is equivalent to the situation that
%% her value is higher than her opponent.\footnote{This trivially holds if the bids functions are strictly increasing at $\bar{\val}$.
%% If there is an interval of valuations $[\val_1,\val_2]$ with the same bids $\bid_1(\bar{\val})$,
%% we can simply consider }
%% Since the allocation is efficient in this case,
%% no trade happens in the secondary market (due to ex post individual rational and ex post budget balance).
%% Thus, we have
%% \begin{align*}
%% \util_1(\bar{\val}) = (\bar{\val} - \bid_1(\bar{\val})) \cdot \Pr_{\val\sim\dist_2}[\val \leq \bar{\val}]
%% = (\bar{\val} - \bid_2(\bar{\val})) \cdot \Pr_{\val\sim\dist_1}[\val \leq \bar{\val}]
%% = \util_2(\bar{\val}).
%% \end{align*}
%% Similarly we also have $\util_1(\bar{\val}') = \util_2(\bar{\val}')$.
%Moreover, by \Cref{lem:payment identity},
%the interim allocations of the agents in the combined market under Bayesian Nash equilibrium satisfy
%\begin{align*}
%u_1(\bar{\val}') - u_1(\bar{\val})
%= \int_{\bar{\val}}^{\bar{\val}'} \tilde{\alloc}_1(\val) \dd \val
%\geq \int_{\bar{\val}}^{\bar{\val}'} \tilde{\alloc}_2(\val) \dd \val
%= u_2(\bar{\val}') - u_2(\bar{\val}).
%\end{align*}
%The inequality holds because (1) the allocation in the auction environment satisfies $\alloc_1(\val) \geq \alloc_2(\val)$ since $\bid_1(\val) > \bid_2(\val)$ for any $\val\in (\bar{\val},\bar{\val}')$;
%and (2) no trade happens in the secondary market if agent $i$ wins the item and $\val_i > \val_{-i}$ since the secondary market satisfies ex post individual rational and weak budget balance.
%The two claims implies that the interim allocation satisfies
%$\tilde{\alloc}_1(\val) \geq \tilde{\alloc}_2(\val)$
%for any $\val\in (\bar{\val},\bar{\val}')$,
%and hence the inequality holds for the integration of the interim allocation.
%Moreover, $\util_1(\bar{\val}) \geq \util_2(\bar{\val})$
%and $\util_1(\bar{\val}') \leq \util_2(\bar{\val}')$
%implies that
%$\util_1(\bar{\val}') - \util_1(\bar{\val})
%\leq \util_2(\bar{\val}') - \util_2(\bar{\val})$,
%and hence both inequalities must hold with equality.
%
%In order for the integral of interim allocations to coincide,
%we have $\tilde{\alloc}_1(\val) = \tilde{\alloc}_2(\val)$ for any $\val\in (\bar{\val},\bar{\val}')$,
%which implies that
%the item is sold from agent $i$ to $-i$ in the secondary market
%if agent $i$ wins the item and $\val_i < \val_{-i}$.
%Therefore, the allocation in the combined market is efficient.
%
%Finally we address the boundary case where the bid of agent $1$ is always above the bid of agent $2$.
%In this case, we know that $u_1(0)\geq u_2(0)$ since
%$u_1(0)\geq 0$ as the utility of agent $1$ is always non-negative under equilibrium,
%and $u_2(0) = 0$ as agent $2$ with value $0$ never wins the item and no trade occurs in the secondary market.
%Moreover, for the highest value $H$, we have $u_1(H) = u_2(H)$.
%First note that under equilibrium we have $b_1(H)=b_2(H)$, because otherwise agent $1$ with value $H$ can decrease her bid and retain the same probability of winning in the auction.
%Since in this case both agents with value $H$ win the item with probability $1$ with payment $b_1(H)=b_2(H)$, and no trade occurs in the secondary market, we have $u_1(H) = u_2(H)$.
%By applying the argument in the previous paragraph,
%the interim allocations for both agents coincide in the combined market,
%and the allocation is efficient.
%
%
%We note that the entire argument is not affect by the signal distribution at all. Thus it is apparent that it does not depend on the content of the signals released after the auction, and in particular, it holds even if the auction bids are revealed before the secondary market.
%\end{proof}

